P-graph Associahedra and Hypercube Graph Associahedra

A graph associahedron is a polytope dual to a simplicial complex whose elements are induced connected subgraphs called tubes. Graph associahedra generalize permutahedra, associahedra, and cyclohedra, and therefore are of great interest to those who study Coxeter combinatorics. This thesis characterizes nested complexes of simplicial complexes, which we call $\Delta$-nested complexes. From here, we can define P-nestohedra by truncating simple polyhedra, and in more specificity define P-graph associahedra, which are realized by repeated truncation of faces of simple polyhedra in accordance with tubes of graphs. We then define hypercube-graph associahedra as a special case. Hypercube-graph associahedra are defined by tubes and tubings on a graph with a matching of dashed edges, with tubes and tubings avoiding those dashed edges. These simple rules make hypercube-graph tubings a simple and intuitive extension of classical graph tubings. We explore properties of $\Delta$-nested complexes and P-nestohedra, and use these results to explore properties of hypercube-graph associahedra, including their facets and faces, as well as their normal fans and Minkowski sum decompositions. We use these properties to develop general methods of enumerating $f$-polynomials of families of hypercube-graph associahedra. Several of these hypercube-graphs correspond to previously-studied polyhedra, such as cubeahedra, the halohedron, the type $A_n$ linear $c$-cluster associahedron, and the type $A_n$ linear $c$-cluster biassociahedron. We provide enumerations for these polyhedra and others.

==> Chapter-3/Chapter-3-Backup-Copy.tex <==

%\usepackage{amsmath}

\chapter{Enumeration Methods}\label{chap:methods}

In this chapter, we aim to establish general methods for enumerating faces of $\p$-associahedra and tubings of $\Delta$-graphs. By enumeration, we wish to find the number of $k$-element tubings of a $\Delta$-graph $G$ for each $k$. When $\Delta$ is dual to a simple polyhedron, this is equivalent to finding the number of co-dimension $k$ faces of the $\p$-graph associahedron of $G$.

%We define two methods in this chapter for enumeration. Both methods work by decomposing $\Delta$-graph tubing complexes into $\Delta$-graph tubing complexes of smaller graphs. This is an inherently recursive process.

We define two separate methods for doing this. When applied to a family of $\p$-graph associahedra, the method outlined in Section \ref{sec:method-one} will enumerate the $f$-polynomials of $\p$-graph associahedra by summing the $f$-polynomials of each facet. These facet $f$-polynomials are found by finding the induced subgraph and reconnected complement of every tube of every $\p$-graph in a family. This method is best applied when this operation of taking reconnected complements is, in some sense, closed; by analogy, the reconnected complement of any tube in a cycle graph is always a cycle, and every tube is a path, whereas the reconnected complement of a tree graph is often not a tree. In the $\p$-graphs studied in this thesis, this method results in a partial differential equation in two variables, and solving this differential equation results in an enumeration of the tubing complexes of these graphs.

The method outlined in Section \ref{sec:method-two} is less straightforward. When applied to a $\p$-graph $G$, it specifies a subset of vertices $X$ of a $\p$-graph, and sorts the tubings of $G$ by cases, according to which tube intersecting with the vertex set $X$ is maximal. This case-by-case method is powerful and is often capable of calculating $f$-polynomials without any differential equations involved. However, it can also require the calculation of $f$-polynomials of several auxiliary $\Delta$-graph associahedra.

In both of these methods, we will establish recursive systems of dependencies. For example, every facet of an associahedron is a product of associahedra, and the first method can be used to define the $f$-polynomials of associahedra. Using the same method, every facet of a cyclohedron is a product of an associahedron and a cyclohedron, and we can define a differential equation relating the $f$-polynomials of cyclohedra and associahedra. As a result, we can calculate $f$-polynomials of $\p$-graph associahedra by relating them to graphs whose $f$-polynomials are known or easier to calculate.

\section{Bivariate $f$-polynomials of families of simplicial complexes}

Define a \emph{power series} to be a symbolic sum $a(s)=\sum_{k\ge 0} a_k s^k$. We say that $a(s)$ expressed as a function for a real number $s$ is a \emph{generating function} of the series $\{a_0,a_1,\ldots\}$. Power series can be defined for multiple variables, such as $a(s,t)=\sum_{k\ge 0} a_{k,n} s^k t^n$. If $a_n(s)=\sum_{k \ge 0} a_{k,n}s^k$, then we can also express $a(s,t)=\sum_{n \ge 0} a_n(s) t^n$.

For a simplicial complex $\Delta$, define the \emph{f-vector} of $\Delta$ to be the vector $(f^\Delta_0,f^\Delta_1, \ldots, f^\Delta_n)$, where $f^\Delta_k$ is the number of faces of $\Delta$ containing $k$ elements. The \emph{f-polynomial} of $\Delta$ is the polynomial $f^\Delta(s) = \sum_{k\ge 0} f^\Delta_k s^k$.

Consider a family of simplicial complexes $\Delta_0, \Delta_1, \ldots$ such that each complex $\Delta_n$ is rank $n$. We define the \emph{bivariate f-polynomial} of this family to be the bi-variate power series $$f^\Delta(s,t) = \sum_{n,k \ge 0} f^{\Delta_n}_k s^k t^n.$$


For a polyhedron $P$, define the \emph{f-vector} of $P$ to be the vector $(f^P_0,\ldots, f^P_n)$, where $f^P_k$ is the number of $k$-dimensional faces of $P$. The \emph{f-polynomial} of $P$ is the polynomial $f^P(x)=\sum_{k\ge 0} f_k^P x^k$.

When $\Delta$ is the dual simplicial complex of an $n$-dimensional simple polyhedron $P$, the f-vectors of $\Delta$ and $P$ are mirror images of each other, with $f^\Delta_k=f^P_{n-k}$ for each $0 \le k \le n$. We then find that $f^P(x)= x^n f^\Delta(x^{-1})$. When $P$ is a simplicial complex with lineality space of dimension $j$, then the dual simplicial complex of $P$ is isomorphic to the dual simplicial complex of the $(n-j)$-dimensional pointed polyhedron, $P / lineal(P)$. We find that $f^P(x) = x^j f^{P/lineal(P)}(x)$, and the first $j$ entries of the $f$-vector of $P$ are zeros. For this reason, we will often find it simpler to work with pointed polyhedra, so that $\Delta(P)$ always has rank equal to the dimension of $P$. \danger{pointed polyhedra mention}

\begin{remark}
Our definition of $f$-vector and $f$-polynomial of a polyhedron $P$ is constructed so as to be dual to the $f$-vector and $f$-polynomial of the dual simplicial complex of $P$. As a result, these $f$-vectors do not have an entry for the $-1$-dimensional face $\emptyset$. This definition varies from definitions for $f$-vectors and $f$-polynomials used in some other publications.
\end{remark}

Consider a family of pointed polyhedra $\{P_0, P_1, \ldots\}$, such that each polyhedron $P_n$ is $n$-dimensional. We define the \emph{bivariate f-polynomial} of this family to be the bi-variate polynomial $$f^P(x,y) = \sum_{n,k \ge 0} f^{P_n}_k x^k y^n.$$

If each polyhedron $P_n$ is dual to a simplicial complex $\Delta_n$, then we note $f_k^{\Delta_n} = f_{n-k}^{P_n}$.
\begin{proposition}

For a family of simple pointed polyhedra $\{P_0,P_1,\ldots\}$ with dual simplicial complexes $\{\Delta_0,\Delta_1,\ldots\}$, we find that defining change of variables $x=1/s$ and $y=st$ gives the equality $$f^P(x,y)=f^\Delta(s,t).$$

\end{proposition}

This allows for equations involving bivariate generating functions of families of simplicial complexes to be applied to families of simple polyhedra.

\begin{proposition}
	For two simplicial complexes $\Delta_1, \Delta_2$, $f^{\Delta_1 \times \Delta_2}(s)=f^{\Delta_1}(s) f^{\Delta_2}(s)$.
\end{proposition}

\begin{proof}
	We note that $\Delta_1 \times \Delta_2$ consists of the union of all faces of $\Delta_1$ and all faces of $\Delta_2$. As a result, every face containing $k$ elements in $\Delta_1 \times \Delta_2$ is the union of a face containing $i$ elements in $\Delta_1$ and $k-i$ elements in $\Delta_2$. This means $f^{\Delta_1 \times \Delta_2}_k = \sum_{i=0}^k f^{\Delta_1}_i f^{\Delta_2}_{k-i}$. As a result of this convolution, $f^{\Delta_1 \times \Delta_2}(s)=f^{\Delta_1}(s) f^{\Delta_2}(s)$.
\end{proof}

\begin{proposition} \label{prop:product-of-polyhedra-f-polynomials}
If $P_1$ and $P_2$ are simple polyhedra, then $f^{P_1 \times P_2}(x)=f^{P_1}(x) f^{P_2}(x)$.
\end{proposition}

\begin{proof}
If $\Delta_1, \Delta_2$ are the dual simplicial complexes of $P_1, P_2$ respectively, with $P_1$ $n$-dimensional and $P_2$ $m$-dimensional, then $$f^{P_1 \times P_2}(x)=x^{n+m}f^{\Delta_1 \times \Delta_2}(1/x)=x^n f^{\Delta_1}(1/x) x^m f^{\Delta_2}(1/x) = f^{P_1}(x) f^{P_2}(x).$$
\end{proof}

%\section{Methods for enumerating faces of nested complexes and nestohedra}

%\subsection{Self-similarity of $\p$-nestohedra}
%
%We know from Proposition \ref{prop:reconnectednestohedra} that every face of a $\p$-nestohedron is itself combinatorially isomorphic to a product of $\p$-nestohedra. We consider this a form of self-similarity among $\p$-nestohedra as a family. However, for certain nestohedra, we see a stronger sense of self-similarity. For instance, every face of the associahedron is combinatorially isomorphic to a product of associahedra, and every face of a cyclohedron is combinatorially isomorphic to a product of associahedra and at most one cyclohedron.
%
%%We can define an equivalent, dual definition for simplicial complexes, stating that a \emph{closed family of simplicial complexes} is one such that every link of an element in each simplicial complex in the family is combinatorially equivalent to the Cartesian product of other simplicial complexes in the family. We can then define a \emph{closed family of polyhedra} is one where the set of dual simplicial complexes of polyhedra in the family is a closed family of simplicial complexes.
%
%\begin{definition}
%A \emph{closed family of $\p$-graphs}, $\mathcal{F}$, is a collection of $\p$-graphs such that, for every $\p$-graph $G$ and tube $t$ of $G$, the simplex-graph $G|_t$ and the $\p$-graph $G/t$ are isomorphic to simplex-graphs and $\p$-graphs in $\mathcal{F}$.
%\end{definition}
%
%In this case, the family of path graphs for all $n$ is a closed family of simplex-graphs. In addition, the family consisting of path graphs and cycle graphs for all $n$ is a closed family of simplex-graphs. The family of all simplex-graphs is also a closed family; however, it is a very large family. We suggest a notion of \emph{small closed families}, such as the family containing path graphs or path and cycle graphs.
%
%We can generalize this notion of closed families to polyhedra.
%
%\begin{definition}
%A \emph{closed family of polyhedra}, $\mathcal{F}$ is a collection of polyhedra such that, for every $P \in \mathcal{F}$, every facet of $P$ is combinatorially isomorphic to the product of two polyhedra in $\mathcal{F}$.
%\end{definition}
%
%The collection of $\p$-graph associahedra of a closed family of $\p$-graphs is a closed family of polyhedra.
%
%If every facet of a polyhedron $P$ is the Cartesian product of polyhedra with known $f$-vectors, then the $f$-vector of $P$ can be calculated. When $P$ is an $n$-dimensional polyhedron in a closed family $\mathcal{F}$, and the $f$-vector of every polyhedron of degree $<n$ in $\mathcal{F}$ is known, then we can calculate the $f$-vector of $P$ through recursion. Subsection \ref{sub:diffeq-method} details a general method for doing this, starting with a more general dual method using simplicial complexes.
%
%%by calculating the $f$-vectors of their facets. If these polyhedra belong to a closed family, then the facets of these polyhedra are products of lower-dimensional polyhedra.

%\section{Bivariate generating functions of families of simplicial complexes and polyhedra}
%
%For a simplicial complex $\Delta$, define the \emph{f-vector} of $\Delta$ to be the vector $(f^\Delta_0,f^\Delta_1, \ldots, f^\Delta_n)$, where $f^\Delta_k$ is the number of faces of $\Delta$ containing $k$ elements. The \emph{f-polynomial} of $\Delta$ is the polynomial $f^\Delta(s) = \sum_{k\ge 0} f^\Delta_k s^k$.
%
%Consider a family of simplicial complexes $\Delta_0, \Delta_1, \ldots$. We define the \emph{bivariate f-polynomial} of this family to be the bi-variate polynomial $$f^\Delta(s,t) = \sum_{n,k \ge 0} f^{\Delta_n}_k s^k t^n.$$
%
%
%For a polyhedron $P$, define the \emph{f-vector} of $P$ to be the vector $(f^P_0,\ldots, f^P_n)$, where $f^P_k$ is the number of $k$-dimensional faces of $P$. The \emph{f-polynomial} of $P$ is the polynomial $f^P(x)=\sum_{k\ge 0} f_k^P x^k$.
%
%\begin{remark}
%Our definition of $f$-vector and $f$-polynomial of a polyhedron $P$ is constructed so as to be dual to the $f$-vector and $f$-polynomial of the dual simplicial complex of $P$. As a result, these $f$-vectors do not have an entry for the $-1$-dimensional face $\emptyset$. This definition varies from definitions for $f$-vectors and $f$-polynomials used in some other publications.
%\end{remark}
%
%Consider a family of polyhedra $P_0, P_1, \ldots$. We define the \emph{bivariate f-polynomial} of this family to be the bi-variate polynomial $$f^P(x,y) = \sum_{n,k \ge 0} f^{P_n}_k x^k y^n.$$
%
%Note that when $\Delta$ is the dual simplicial complex of a simple polyhedron $P$, the f-vectors of $\Delta$ and $P$ are mirror images of each other, with $f^\Delta_k=f^P_{n-k}$. In addition, if $P$ is $n$-dimensional, then $f^P(x)= x^n f^\Delta(x^{-1})$, and vice-versa.
%
%For a family of simple polyhedra $\{P_0,P_1,\ldots\}$ with family of dual simplicial complexes $\{\Delta_0,\Delta_1,\ldots\}$, we find that if we define a change of variables $x=1/s$ and $y=st$, we have the equality $$f^P(x,y)=f^\Delta(s,t).$$
%
%This allows for equations involving bivariate generating functions of families of simplicial complexes to be applied to families of simple polyhedra.
%
%\begin{proposition}
%	For two simplicial complexes $\Delta_1, \Delta_2$, $f^{\Delta_1 \times \Delta_2}(s)=f^{\Delta_1}(s) f^{\Delta_2}(s)$.
%\end{proposition}
%
%\begin{proof}
%	We note that $\Delta_1 \times \Delta_2$ consists of the union of all faces of $\Delta_1$ and all faces of $\Delta_2$. As a result, every face containing $k$ elements in $\Delta_1 \times \Delta_2$ is the union of a face containing $i$ elements in $\Delta_1$ and $k-i$ elements in $\Delta_2$. This means $f^{\Delta_1 \times \Delta_2}_k = \sum_{i=0}^k f^{\Delta_1}_i f^{\Delta_2}_{k-i}$. As a result of this convolution, $f^{\Delta_1 \times \Delta_2}(s)=f^{\Delta_1}(s) f^{\Delta_2}(s)$.
%\end{proof}
%
%\begin{proposition}
%If $P_1$ and $P_2$ are simple polyhedra, then $f^{P_1 \times P_2}(x)=f^{P_1}(x) f^{P_2}(x)$.
%\end{proposition}
%
%\begin{proof}
%If $\Delta_1, \Delta_2$ are the dual simplicial complexes of $P_1, P_2$ respectively, with $P_1$ $n$-dimensional and $P_2$ $m$-dimensional, then $$f^{P_1 \times P_2}(x)=x^{n+m}f^{\Delta_1 \times \Delta_2}(1/x)=x^n f^{\Delta_1}(1/x) x^m f^{\Delta_2}(1/x) = f^{P_1}(x) f^{P_2}(x).$$
%\end{proof}

%Define the \emph{bivariate $f$-polynomial} of this family of polyhedra to be the bivariate polynomial $$f(x,y) = \sum_{n,k \ge 0} f^{\Delta_n}_k s^k t^n.$$



%\subsection{Facially isomorphic polyhedra}
%
%The \emph{lineality space} $lineal(P)$ of a polyhedron $P$ in vector space $V$ is the linear subspace of $V$ such that $v$ is in the lineality space of $P$ if and only if $x+v \in P$ for all $x \in P$. We know that the lineality space of a pointed polyhedron is the space $\{0\}$. We know that $P \cong (P/lineal(P))\times lineal(P)$.
%
%We should note that $P$ and $P/lineal(P)$ both have isomorphic dual simplicial complexes. For any simple polyhedron $P$, the rank of $\Delta(P)$ will be equal to the dimension of $P/lineal(P)$. 
%
%\begin{definition}
%The \emph{apparent dimension} of a simple polyhedron is the dimension of $P/lineal(P)$.
%\end{definition}
%
%Because we perform our calculations using the dual simplicial complexes of polyhedra, and they hypercube case relies heavily on manipulations of forbidden subset diagrams which reflect the dual simplicial complexes of polyhedra, this means it is in our interest to index families of polyhedra by their apparent dimension. We should note the following: if $P$ is an $n$-dimensional polyhedron of apparent dimension $n-\rho$, then $f^P(x) y^n = x^k y^k f^{P/lineal(P)}(x)$. 

\section{Atomic link sum polynomial method for enumerating $f$-polynomials}\label{sec:method-one}

In introducing this section, we first provide a simplified version of the algorithm defined in this section. In a simple $n$-dimensional polyhedron, every vertex is contained in $n$ facets. As a result, we can count the number of vertices in an $n$-dimensional polyhedron by counting the number of vertices in each facet, adding the vertex counts for each facet together, and then dividing by $n$. If we are counting the number of vertices in a $\p$-nestohedron using this method, it helps to recall that according to Theorem \ref{thm:reconnectednestohedra1}, every facet of a $\p$-nestohedron is isomorphic to the product of two lower-dimensional $\p$-nestohedra. Also, according to Proposition \ref{prop:product-of-polyhedra-f-polynomials}, the number of vertices in the product of two polyhedra is isomorphic to the product of vertices in each polyhedron. As a result, we can calculate the number of vertices in each facet $\Phi_I$ of a $P$-nestohedron $\nest{P}{\B}$ by rewriting it as the product of two polyhedra, the simplex-nestohedron of $\B$ restricted to $I$, and the $F_I$-nestohedron of the building set $\B/I$. After finding the number of vertices of each nestohedron, we take the product and find the number of vertices in the facet $\Phi_I$. After finding the number of vertices in each facet $\Phi_I$ of the nestohedron $\nest{P}{\B}$, we sum the values up and divide by $n$.

The enumeration method outlined in this section introduces two complications to this method. First of all, every simple polyhedron is dual to a simplicial complex, and so we can get more general results by proving everything for enumeration of maximal faces in simplicial complexes. Second of all, we wish to enumerate not only the vertices of simple polyhedra, but instead enumerate all $k$-dimensional faces. We can do this by taking products of bivariate $f$-polynomials.

%\subsection{Miniature Example: Counting faces of a cube}
%
%As a loose introduction to this section, consider the counting of the faces of a three-dimensional cube. If we know that a cube has 6 square facets, and each square has 4 vertices, then adding up the number of vertices in each facet gives us 24 vertices. However, each vertex is contained in 3 facets. Therefore, we overcount by a factor of 3 and must divide to find that a cube contains 8 vertices. This can be extended to all faces by noting that each edge appears in 2 facets, each 2-dimensional face appears in 1 facet, and so on. If $f$ is the $f$-vector of a cube and $g$ is the sum of $f$-vectors of facets of a cube, we find that $g=(3f_0,2f_1,1 f_2, 0 f_3)$.
%
%This section introduces a broad generalization of this counting method, with a few major complications. First, we will find that the relationship $g=(3f_0,2f_1,1 f_2, 0 f_3)$ in the prior example can be rewritten for bi-variate $f$-polynomials of any dimension, and that this form of element-wise multiplication will correspond to a differential equation relating power series.
%Secondly, we are developing this theory for the case where $P$ is a $\p$-graph associahedron. As a result, every facet of $P$ is a product of $\p$-graph associahedra $A$ and $B$.
%Thirdly, our example with the cube took advantage of the fact that every facet is isomorphic, but we will need to carefully count how many facets of what type each polyhedron contains.
%Finally, we remember that if a simple polyhedron $P$ is dual to a complex $\Delta$, then each facet of $P$ is dual to the link of a singleton element in $\Delta$. As a result, we will do our calculations first in terms of simplicial complexes, and then at the end of the section we will translate these results in terms of simple polyhedra, which is the case we are most interested in.
%
%%As a very basic example of the motivation of this method, consider the enumeration of sets in a Boolean lattice. A Boolean lattice on $3$ elements has f-vector $(1,3,3,1)$.
%
%\danger{Introduction to the concept with an example?}

%\subsection{Naive method: Cyclohedron}
%
%The general method presented in the next subsection is very general. We will provide an specific example here.
%
%Consider a cycle graph on $n+1$ vertices. The simplex-graph associahedron of this graph is the cyclohedron, $B_n$. Write $f^B_{n,k}$ to be the number of $k$-dimensional faces of the $n$-dimensional cyclohedron.
%
%For a cyclohedron $B_n$, we wish to sum up the $f$-vectors of every facet of $B_n$. Once we know this sum, we will be able to determine the $f$-vector of $B_n$ itself.
%
%Every facet $\Phi_t$ of an $n$-dimensional cyclohedron is in bijection with a tube $t$ of the cycle graph $G$ on $n+1$ vertices. The face $\Phi_t$ is combinatorially isomorphic to the product of the simplex-graph associahedron of the graph $G|_t$ and the simplex-graph associahedron of the graph $G/t$. If $t$ is a tube on $i+1$ vertices, then $G|_t$ is a path graph on $i+1$ vertices, and $G/t$ is a cycle graph on $n-i$ vertices. If $A_i$ is the $i$-dimensional associahedron, then we find that the $f$-vector of this facet is equal to $f^{A_i}(x) f^{B_{n-1-i}}(x)$.
%
%For each $0 \le i \le n-1$, there are $n+1$ tubes in the cycle graph containing $i+1$ vertices. As a result, the sum of $f$-polynomials of facets of $B_n$ is equal to
%
%\[
%	\sum_{i=0}^{n-1} (n+1) f^{A_i}(x) f^{B_{n-1-i}}(x)
%\]
%
%If $F$ is a $k$-dimensional face of $B_n$, then because $B_n$ is simple, $F$ is contained in $n-k$ facets of $F$. We can then write that this facet sum polynomial is equal to the polynomial
%
%\[
%	\sum_{i=0}^n f^{B_n}_k (n-k) x^k.
%\]
%
%As a reminder, if $g(x)=\sum_{n\ge 0} g_n x^n$, then $\sum_{n \ge 0} n g_n x^n = xD_x g(x)$, where $D_x g(x) = g'(x)$. This means the facet sum polynomial is equal to
%
%\[
%	n f^{B_n}(x) - x D_x f^{B_n}(x).
%\]
%
%
%
%For each dimension $n$, we find a differential equation involving $f^{B_n}(x)$ and lower-dimensional $f$-polynomials.
%
%\[
%	n f^{B_n}(x) - x D_x f^{B_n}(x) = \sum_{i=0}^{n-1} (n+1) f^{A_i}(x) f^{B_{n-1-i}}(x)
%\]
%
%We can use multivariate $f$-polynomials to sum over all $n$. Multiply each side of the equation by $y^n$, and sum over all $n \ge 0$. On the left hand side, we get
%
%\[
%	\left[\sum_{n \ge 0} n f^{B_n}(x)y^n\right] - x D_x \sum_{n=0} \left[f^{B_n}(x)y^n\right]
%\]
%
%which we can rewrite as
%
%\[
%	y D_y f^B(x,y) - x D_x f^B(x,y).
%\]
%
%The right hand side of the equation is equal to
%
%\[
%	y\sum_{n\ge 0} \sum_{i=0}^{n-1} (n+1) f^{A_i}(x) y^i f^{B_{n-1-i}}(x) y^{n-1-i}
%\]
%
%Splitting $(n+1)=(i)+(n-1-i)+(2)$ allows us to rewrite this as
%
%	\[y\sum_{n\ge 0} \sum_{i=0}^{n-1} \left[ i f^{A_i}(x) y^i f^{B_{n-1-i}}(x)y^{n-1-i}\right] +\left[ f^{A_i}(x) y^i (n-1-i) f^{B_{n-1-i}}(x)y^{n-1-i}\right]\] \[+\left[ 2f^{A_i}(x) y^i f^{B_{n-1-i}}(x)y^{n-1-i}\right]\]
%
%Isolating the sum of all terms in the first bracket and applying a convolution formula gives
%
%\[
%	\sum_{n \ge 1} \sum_{i=0}^{n-1} i f^{A_i}(x) y^i f^{B_{n-1-i}} = \left[\sum_{n \ge 0} n f^{A_n}(x) y^n\right] \left[ \sum_{n \ge 0} f^{B_n}(x)y^n\right]
%\]
%
%This becomes $\left[y D_y f^{A}(x,y)\right] f^B(x,y)$. Applying convolution formulas to the second two terms and plugging the left hand side of the equation back in gives the following differential equation; for compactness of form, we have written $f^A(x,y)=f^A$ and $f^B(x,y)=f^B$.
%
%\[
%	y D_y f^B - x D_x f^B = y \left[(yD_yf^A) f^B + f^A (yD_y f^B) + 2 f^A f^B\right]
%\]
%
%This is a partial differential equation relating $f^A(x,y)$ and $f^B(x,y)$, and can be used to verify $f^B(x,y)$ if $f^A(x,y)$ is known.

\subsection{Atomic link sum polynomial method for enumerating $f$-polynomials of simplicial complexes}

An atomic element of a poset with minimal element is an element which covers the minimal element. The atomic elements of a simplicial complex are the singleton set faces of that simplicial complex, and so we call the link of a singleton face of a simplicial complex an \emph{atomic link}.

Define the \emph{atomic link sum polynomial} of a simplicial complex $\Delta$ to be the sum

\[
	R^\Delta(s) = \sum_{x \in \mathcal{S}} f^{\Delta / \{x\}} (s)
\]

of $f$-polynomials of the links of every singleton subset of the base set $\mathcal{S}$ of $\Delta$. For every face $S$ of $\Delta$ with $|S| \ge 1$, there is a face $S \backslash \{x\}$ in $\Delta/\{x\}$ for each $x \in S$. We note then that for every $k \ge 1$, there is a one-to-$k$ correspondence between $k$-dimensional faces of $\Delta$ and $(k-1)$-dimensional faces of $\Delta/\{x\}$ for any $x \in \mathcal{S}$. This means that $\sum_{x \in \mathcal{S}} f^{\Delta/\{x\}}_k= k f_{k+1}^\Delta$ for all $k \ge 1$. As a result, we write $R^\Delta(s) = f_1^\Delta+2f_2 ^\Delta s + 3 f_3^\Delta s^2 + \cdots$. This can be reduced to a derivative:

\[
	R^\Delta (s) = D_s f^\Delta(s),
\]
where $D_s$ is the differential operator representing the derivative with respect to $s$. When $\Delta$ is a family $\{\Delta_0,\Delta_1,\ldots\}$, we define $R^\Delta(s,t)=\sum_{n\ge 0} R^{\Delta_n}(s) t^n$.



\bigskip



Consider a set of families of simplicial complexes $A^\sigma=\{A^\sigma_0, A^\sigma_1,\ldots\}$,  $B^\sigma = \{B^\sigma_0,B^\sigma_1,\ldots\}$, indexed by $n \ge 0$ and $\sigma$ in a set $S$. We call each $\sigma \in S$ a \emph{shape}. We say that a family $\Delta$ of simplicial complexes $\{\Delta_0, \Delta_1, \ldots\}$ is \emph{atomically closed under $A$ and $B$} if for each simplicial complex $\Delta_n$, every atomic link of $\Delta_n$ is isomorphic to the product $A_i^\sigma \times B^\sigma_{n-1-i}$ for some shape $\sigma$ in $S$ and $i \in \{0,\ldots,n-1\}$.% Most importantly, for every atomic link $L$ of $\Delta_n$, $f^L(s)=f^{A_i^\sigma}(s) \times f^{B_{n-1-i}^\sigma}(s)$.



Consider a family of simplicial complexes $\Delta=\{\Delta_0,\Delta_1,\ldots\}$ which is atomically closed under $A$ and $B$. In the case that some atomic link can be expressed as such a product in more than one way, express it as a canonical product using a unique pair $(i,\sigma)$. Now define $r_\sigma(n,i)$ to be the number of atomic links of $\Delta_n$ which can be canonically expressed as a product $A_i^\sigma \times B_{n-1-i}^\sigma$. We find that the $f$-polynomial of $A_i^\sigma \times B_{n-1-i}^\sigma$ is equal to the product $f^{A_i^\sigma}(s) \times f^{B_{n-1-i}^\sigma}(s)$. As a result, we find

\[
	R^{\Delta_n} (s) = \sum_{\sigma \in S} \sum_{i=0}^{n-1} r_\sigma(n,i) f^{A_i^\sigma}(s) \times f^{B_{n-1-i}^\sigma}(s) .
\]

Multiplying by $t^n$ for each $n$ and summing over all $n\ge 0$ gives the following.

\[
	R^\Delta(s,t) =  \sum_{n \ge 0} \sum_{\sigma \in S} t \sum_{i=0}^{n-1} r_\sigma(n,i) f^{A_i^\sigma}(s)t^i \times f^{B_{n-1-i}^\sigma}(s) t^{n-1-i}.
\]



%Consider the case where $\Delta_0,\Delta_1, \ldots$ is a sequence of simplicial complexes, and there is a set of simplicial complexes $A^\sigma_n, B^\sigma_n$ indexed by shape $\sigma \in S$ and $n \in \mathbb{N}$. Consider the case that every atomic link in $\Delta_n$ is isomorphic to the product of two simplicial complexes $A^\sigma_i \times B^\sigma_{n-1-i}$. Furthermore, the $f$-polynomial of $A^\sigma_i \times B^\sigma_{n-1-i}$ is $f^{A^\sigma_i}(s) \times f^{B^\sigma_{n-1-i}}(s)$. If we can enumerate that for $\Delta_n$, there are $r_\sigma(n,i)$ atomic links of type $A^\sigma_i \times B^\sigma_{n-1-i}$, we find that the bivariate atomic link sum polynomial is equal to
%
%\[
%	\sum_{\sigma \in S} \sum_{i=0}^{n-1} r_\sigma(n,i) f^{A^\sigma_i}(s) \times f^{B^\sigma_{n-1-i}}(s) t^n
%\]

Consider the case that $r_\sigma(n,i)$ can be written as a sum of functions separable in $i,n-1-i$, of the form \[r_\sigma(n,i) = \sum_{j=1}^k r_\sigma^{A,j}(i) r_\sigma^{B,j}(n-1-i).\]

In this event, we can express the sum $R^\Delta(s,t)$ as

\[
	R^\Delta(s,t) = \sum_{n \ge 0} \sum_{ \sigma \in S}\sum_{j \ge 1}^k t \sum_{i=0}^{n-1} \left[r^{A,j}_\sigma(i) f^{A_i^\sigma}(s)t^i\right] \times \left[r^{B,j}_\sigma (n-1-i)f^{B_{n-1-i}^\sigma}(s) t^{n-1-i}\right]
\]

	This is a convolution of the power series $r_\sigma^{A,j}(n) f^{A^\sigma_n}(s)t^n$ and $r_\sigma^{B,j}(n) f^{B^\sigma_n}(s)t^n$. As a result, we can rewrite

\[
	R^\Delta(s,t) = \sum_{j =1}^k \sum_{\sigma \in S} t \left( \sum_{n\ge 0} r_\sigma^{A,j}(n) f^{A^\sigma_n} (s) t^n\right)
\left( \sum_{n\ge 0} r_\sigma^{B,j}(n) f^{B^\sigma_n} (s) t^n\right) .
\]

Given a power series $a(t)=\sum_{n \ge 0} a_n t^n$, define $O_t^r$ to be the linear operator on power series defined by $O_t^r\left[a(t)\right]\sum_{n\ge 0} r(n) a_n t^n$.  To simplify notation and avoid nested scripts, we will define $O_t^{A,\sigma,j}=O_t^{r^{A,j}_\sigma}$. Noting that $R^\Delta(s,t)=D_s f^{\Delta}(s,t)$, we can now arrive at a final equation.

\begin{proposition} \label{prop:diff-eq}
For a family $\Delta$ of simplicial complexes atomically closed under $A$ and $B$, with counting function $r_\sigma(n,i)$ separable into functions of the form $r_{\sigma}^{A,j}(i)$ and $r_{\sigma}^{B,j}(n-1-i)$ and defining linear operators $O_t^{A,\sigma,j}$ and $O_t^{B,\sigma,j}$ on power series, the following partial differential equation holds:
\[
	D_s f^{\Delta} (s,t) = t \sum_{\sigma \in S}\sum_{j=1}^k O^{A,\sigma,j}_t\left[f^{A^\sigma}(s,t)\right] O_{t}^{B,\sigma,j} \left[f^{B^\sigma}(s,t)\right]
	.
\]

\end{proposition}

We should note that for a family of simplicial complexes, we assume $f^{\Delta_n}_0=1$ for each $n \ge 0$. This allows us to create a boundary condition to solve this as a differential equation.

\begin{remark}
For many functions $r(n)$, the linear operator $O_t^r$ is fairly simple. For instance, when $r(n)=\delta(n)$, the function such that $\delta(n)=1$ if and only if $n=0$ and $0$ otherwise, we find $O_t^r[a(t)]=a(0)$. When $r(n)=n$, we find $O_t^r[a(t)]=t D_t [a(t)]$. Finally, $O_t^{rs}=O_t^r O_t^{s}$ and $O_t^{r+s}=O_t^r + O_t^s$, so we can calculate $O_t^r$ easily whenever $r$ is a polynomial or the $\delta$ function. We also note that $O_t^{\delta(n-i)}[a(t)]=a^{(i)}(0)/i!$.
\end{remark}

Now we can restate this for simple polyhedra. In the event that each simplicial complex in $\Delta, A$, and $B$ of rank $n$ is isomorphic to the dual simplicial complex of an $n$-dimensional pointed simple polyhedron, we can perform a change of variables $x=1/s, y=st$ and note that $f^{\Delta}(s,t)=f^{P(\Delta)} (x,y)$. Performing this change of variables allows us to reformulate an earlier expression:

\[
	D_s f^\Delta(s,t) = \sum_{\sigma \in S} \sum_{j=1}^k xy \left(r^{A,j}_\sigma(n) f^{P(A^\sigma_n)}(x)y^n\right)
	\left(r^{B,j}_\sigma(n) f^{P(B^\sigma_n)}(x)y^n\right).
\]



We can rewrite this using the same linear operator on power series $O_y^{A,\sigma,j}$, this time using the variable $y$ instead of $t$. It should be emphasized that one does not need to re-calculate these linear operators beyond replacing every use of $t$ with $y$.

We can also rewrite $D_s f^\Delta(s,t)=xy D_y f^{P(\Delta)}(x,y)-x^2 D_x f^{P(\Delta)}(x,y)$. After dividing by $y$, we can finally write the equation as follows.

\begin{proposition} \label{prop:diff-eq-polyhedra}
When each simplicial complex in $\Delta, A,$ and $B$ from Proposition \ref{prop:diff-eq} is dual to a pointed simple polyhedron, the following differential equation holds:
\[
	(yD_y -x D_x) f^{P(\Delta)}(x,y) = \sum_{\sigma \in S} \sum_{j =1}^k y O^{A,\sigma,j}_y \left[f^{P(A^\sigma)}(x,y)\right]O^{B,\sigma,j}_y\left[f^{P(B^\sigma)}(x,y)\right].
\]
\end{proposition}

\subsection{$\p$-graph case}

The definition of atomically-closed families of simplicial complexes is inspired by self-similarity of associahedra and graph associahedra. Recall that every facet of a $\p$-graph associahedron is combinatorially isomorphic to the product of the associahedron of a $\p$-graph $G/t$ and a simplex-graph associahedron $G|_t$. Say that a family of $\p$-graphs $G=\{G_0,G_1,\ldots\}$ is \emph{facet-closed} under $\p$-graph families $A$ and $B$ indexed by $n$ and $\sigma$ if, for every tube $t \in G_n$, the simplex graph $G|_t$ is isomorphic to a simplex-graph in $A$ and the reconnected complement of $t$ is isomorphic to a $\p$-graph in $B$. We also say that the families of their $\p$-graph associahedra are also facet-closed.

We take note of some well-known facet-closed families of graph associahedra. The associahedron is a the simplex-graph associahedron of a path graph. Every tube of a path graph induces a path graph, and the reconnected complement is a path graph, so we say that path simplex-graphs are facet-closed under path simplex-graphs and path simplex-graphs, and associahedra are facet-closed under associahedra. Alternatively, every facet of a cyclohedron is isomorphic to the product of a cyclohedron and an associahedron, so it is facet-closed under the families of associahedra and cyclohedra. For a much larger family, consider the set of all $\p$-graphs. Every facet of a $\p$-graph associahedron is the product of lower-dimensional $\p$-graph associahedra, and so this set of graphs is facet-closed if we choose a shape set $S$ with infinite possible shapes.

There are three features in families of graphs which make them good candidates for atomic link sum enumeration. First, we wish for a small number of possible tube shapes. Secondly, we look for self-similarity; if a family decomposes into families $A$ and $B$, and $\Delta$ is one of the families $A^\sigma$ or $B^\sigma$, then this is still an equation involving $f^\Delta$. Thirdly, we hope that $O_t^{A,\sigma,j}$ and $O_t^{B,\sigma,j}$ can be rewritten using the derivative operator $D_t$ and the evaluation operator. Specifically, if $r_\sigma^{A,j}$ and $r_\sigma^{B,j}$ can be written as polynomials, or are delta functions of the form $\delta(n-i)$, then the resulting operators are easy to compute. For example, if $r(n)=n$, then $O_t^r[a(t)]=t D_t [a(t)]$, and if $r(n)=n^k$, then $O_t^r[a(t)]=(tD_t)^k a(t)$. Define $\delta(t)$ to be the function where $\delta(0)=1$ and $\delta(i)=0$ for all $i \ne 0$. We find $O_t^\delta[a(t)]=a(0)$, and $O_t^{\delta(n-i)}[a(t)]=a^{(i)}(t)/i!$. These delta functions are useful in the case when a tube or its complement only occurs at a certain size. %In the event that a function $r^{A,j}_\sigma(n)$ contains a term $n!$, it may be advisable to convert to exponential generating functions, but other than cases where graphs are a variation upon a complete graph, we have not found much use for them.

%Now consider the $\p$-graph case. Consider a family of graphs $G=\{G_0,G_1,\ldots\}$. Assume that the family of tubing complexes of $G$ is atomically closed, into tubing complexes of graphs of the families $A^\sigma$, $B^\sigma$, with shapes $\sigma \in S$. Count $r_\sigma(n,i)$ to be the number of tubes of shape $\sigma$ in $G_n$ containing $i+1$ vertices. This is an enumerative problem and will be unique to each graph. We see that $G|_t\cong A_i^\sigma$ and $G/t \cong B_{n-1-i}^\sigma$. If possible, we rewrite $r_\sigma(n,i)$ into sums of separable functions of the form $r_\sigma^{A,j}(i) r_\sigma^{B,j}(n-1-i)$, and use these to define the linear operators $O_t^{A,\sigma,j}$ and $O_t^{B,\sigma,j}$.


\begin{proposition}
Consider a family of simplicial complexes $\Delta=\{\Delta_0,\Delta_1,\ldots\}$ and a collection of $\Delta$-graphs $G=\{G_0,G_1,\ldots\}$ such that each graph $G_n$ is a $\Delta_n$-graph. Say that a family of graphs $G$ decomposes into families of graphs $A$ and $B$, such that for every tube shape $\sigma$ in graph $G_n$, there are $r_\sigma(n,i)$ tubes $t$ of $G_n$ of shape $\sigma$ containing $i$ elements, such that each tube $t$ induces a graph isomorphic to $A_i^\sigma$ in $G_n$, and the reconnected complement of $t$ in $G_n$ is a graph isomorphic to $B_{n-1-i}^\sigma$. Assume that each $r_\sigma(n,i)$ is separable into a finite sum of products of functions of the form $r^{A,j}_\sigma$ and $r^{B,j}_\sigma$. If $f^G, f^{A^\sigma}, f^{B^\sigma}$ are taken as the bivariate $f$-polynomials of the nested complexes of the respective families of graphs, we find the following:
\[
	D_s f^{G} (s,t) = t \sum_{\sigma \in S}\sum_{j=1}^k O^{A,\sigma,j}_t\left[f^{A^\sigma}(s,t)\right] O_{t}^{B,\sigma,j} \left[f^{B^\sigma}(s,t)\right].
\]
\end{proposition}

The following is a restatement of this proposition for the $\p$-graph case.

\begin{proposition}
Consider a family of simple pointed polyhedra $P=\{P_0,P_1,\ldots\}$ such that each polyhedron $P_n$ is $n$-dimensional, and a family of $P$-graphs $G=\{G_0,G_1,\ldots\}$ such that each graph $G_n$ is a $P_n$-graph. Say that a family of graphs $G$ decomposes into families of $\p$-graphs $A$ and $B$ indexed by variables $n\ge 0$ and shape $\sigma$, such that for every tube $t$ of shape $\sigma$ in graph $G_n$ with $|t|=i+1$, the simplex-graph $G_n|_t$ is isomorphic to the simplex-graph $A_i^\sigma$, and the reconnected complement of $t$ in $G_n$ is a $F_t$-graph isomorphic to the $\p$-graph $B_{n-1-i}^\sigma$. Assume that each $r_\sigma(n,i)$ is separable into a finite sum of products of functions of the form $r^{A,j}_\sigma$ and $r^{B,j}_\sigma$. If $f^G, f^{A^\sigma}, f^{B^\sigma}$ are taken as the bivariate $f$-polynomials of the $\p$-graph associahedra of their respective families of graphs, we find the following:
\[
(yD_y -x D_x) f^{G}(x,y) = \sum_{\sigma \in S} \sum_{j =1}^k y O^{A,\sigma,j}_y \left[f^{A^\sigma}(x,y)\right]O^{B,\sigma,j}_y\left[f^{B^\sigma}(x,y)\right].
\]
\end{proposition}

. %In the special hypercube cases studied in this paper using this method, we have found that each equation can be written as a partial differential equation.

%This section also introduces a simplicial complex operation called vertex deletion, where a subset from the base set of a simplicial complex is removed, and all faces which intersected with this deleted set are removed. The dual operation on simple polyhedra is the deletion of a set of facets, and to help understand the implications of this construction, we introduce the concept of half-open polyhedra in Subsection \ref{sub:halfopen}.

%
%
%%Viewing each part of this product as a power series in $t$, we see the map taking power series $\sum_{n \ge 0} f^{A^\sigma_n}(s)t^n$ to power series $\sum_{n\ge 0} r_\sigma^A(n) f^{A^\sigma_n}(s) t^n$ is a \emph{linear operator} in $t$ on the set of formal power series on $\R[s]$. Write this linear operator as $O_t^{A^\sigma}$, and define $O_t^{B^\sigma}$ in a similar manner. We know that every linear operator on $t$ can be rewritten in the form $\sum_{n \ge 0} \mathfrak{M}(p_n) D_t^n$, where $\mathfrak{M}(p_n)$ is the linear operator representing multiplication by a polynomial $p_n$.
%
%\danger{I read this for polynomials, but it might only be true for polynomials and not power series... we might say that for all of the example cases used in this paper, the linear operators found have been of this form.} This expression can now be simplified as follows.
%
%%\begin{theorem}
%%A linear operator on the ring of formal power series on $\R[x]$ is an endomorphism on the ring of formal power series, and can be written as a sum $\sum_{n \ge 0} \mathfrak{m}(p_n) D_x^n$, where $\mathfrak{m}(p_\alpha)$ is the operator representing multiplication by the polynomial $p_\alpha$, and $D_x$ is the differential operator on $x$. \danger{Am I thinking of just finite operators? eesh...}
%%\end{theorem}
%%
%%Note that when 
%%
%%\danger{Let's write the operators $O^{A^\sigma}_t [f^{A^\sigma}(s)] = \sum_{n \ge 0} r_\sigma^A(n) f^{A^\sigma_i}(s) t^n$. It is an operator on $f^{A^\sigma_i}$.}
%
%\[
%	D_s f^{\Delta} (s,t) = \sum_{\sigma \in S} t O^{A^\sigma}_t\left[f^{A^\sigma}(s,t)\right] O_{t}^{B^\sigma} \left[f^{B^\sigma}(s,t)\right]
%\]
%
%We can rewrite a dual expression of this equation for the case where each simplicial complex belonging to a family $\Delta, A^\sigma, B^\sigma$ is polyhedral. We note that in this case, for each shape $\sigma$, there will be $r_\sigma(n,i)$ facets of $P(\Delta_n)$ of type $P(A_i^\sigma) \times P(B_{n-1-i}^\sigma)$. For a sequence $\{\Delta_0,\Delta_1, \ldots\}$ of simplicial complexes dual to simple polyhedra $\{P(\Delta_0), P(\Delta_1), \ldots\}$ with each polyhedron $P(\Delta_n)$ being $n$-dimensional, we know from the duality of bivariate $f$-polynomials that $f^{\Delta}(s,t)=f^{P(\Delta)}(x,y)$ when $x=1/s$ and $y=st$. This will allow us to make a statement about the bivariate generating function for the family of polyhedra $P(\Delta)$. Replacing some of the terms gives
%
%\[
%	D_s f^\Delta(s,t) = \sum_{\sigma \in S} xy \left(r^A_\sigma(n) f^{P(A^\sigma_n)}(x)y^n\right)
%	\left(r^B_\sigma(n) f^{P(B^\sigma_n)}(x)y^n\right).
%\]
%
%Application of the chain rule finds that $D_s f^\Delta(s,t) = xy D_y f^{P(\Delta)}(x,y) - x^2 D_x f^{P(\Delta)}(x,y)$. Using this, we can rewrite both sides of this equation and simplify by dividing by $x$. Now, note that $O^{A^\sigma}_t$ and $O^{B^\sigma}_t$ are both determined by the form of $r^A_\sigma$ and $r^B_\sigma$, expressed as operations on generating functions. Because this new equation has the same form, we find we can rewrite this equation by using operators $O^{A^\sigma}_y$ and $O^{B^\sigma}_y$, obtained by switching the variable but not the form of each operator. Rewriting the equation in this way gives us the new differential equation relating bivariate $f$-polynomials of polyhedra.
%
%\[
%	yD_y f^{P(\Delta)}(x,y)-x D_x f^{P(\Delta)}(x,y) = \sum_{\sigma \in S} y O^{A^\sigma}_y \left[f^{P(A^\sigma)}(x,y)\right]O^{B^\sigma}_y\left[f^{P(B^\sigma)}(x,y)\right]
%\]

%\subsection{Differential equations derived from bivariate $f$-polynomials of atomic links} \label{sub:diffeq-method}
%
%
%
%%The primary aim of this subsection is to generalize the enumeration method used in the last subsection for all $\p$-graph associahedra, and provide a framework for the work done in Chapter \ref{chap:res2}. This is done by generalizing for a special case of simplicial complexes, and then providing an outline for applying this method to $\p$-graph associahedra. Note that while all tubes of a cycle graph induce path graphs, and all reconnected complements are cycle graphs, tubes for other graphs come in multiple `shapes.' As a result, we will have to repeat this process for multiple different shapes of tube. 
%
%The primary aim of this subsection is to generalize the enumeration method used in the last subsection for all $\p$-graph associahedra, and provide a framework for the work done in Chapter \ref{chap:res2}.
%
%This is a good time to reflect on how to apply this method to other $\p$-graph associahedra. First of all, in the cycle graph, all tubes induce path subgraphs, and all reconnected complements are cycle graphs. This is not the case in all graphs, where induced subgraphs can take on many forms. We must sort tubes of a $\p$-graph $G$ into `shapes' $\sigma_1, \ldots, \sigma_k$ such that, if $t_1, t_2$ have shape $\sigma_i$ and $|t_1|=|t_2|$, then $G_{t_1} \cong G_{t_2}$ and $G/t_1 \cong G/t_2$.
%
%Now, write $\sigma$
%
%Define an \emph{atomic link} as the link of an atomic element in a simplicial complex. Define the \emph{atomic link sum polynomial} of a simplicial complex $\Delta$ to be the sum
%
%\[
%	R^\Delta(s) = \sum_{x \in \mathcal{S}} f^{\Delta / \{x\}} (s)
%\]
%
%of $f$-polynomials of the links of every singleton subset of the base set $\mathcal{S}$ of $\Delta$. For every $k$-element set $S$ in $\Delta$, the atomic link sum polynomial counts $k$ sets of the form $S \backslash \{i\}$ for $i\in S$. As a result, we find $R^\Delta(s) = f_1^\Delta+f_2 ^\Delta s + 3 f_3^\Delta s^2 + \cdots$. This can be reduced to a derivative:
%
%\[
%	R^\Delta (s) = D_s f^\Delta(s),
%\]
%where $D_s$ is the differential operator representing the derivative with respect to $s$.
%
%
%For a family of simplicial complexes $\Delta=\{\Delta_0,\Delta_1,\ldots\}$, consider the case where there exists two sets of simplicial complexes, each complex $A^\sigma_i$ and $B^\sigma_i$ indexed by $i \in \mathbb{N}$ and $\sigma$ in a finite set $S$, such that each atomic link of $\Delta_n$ is isomorphic to the Cartesian product of $A^\sigma_i \times B^\sigma_{n-1-i}$ for some $\sigma \in S$ and some $i \in \mathbb{N}$. We call $S$ the set of \emph{shapes} of the atomic link.
%
%We can categorize each atomic link of a simplicial complex $\Delta_n$ as being of a single type $A_i^\sigma \times B^{\sigma}_{n-1-i}$ for some shape $\sigma$ and $i\in\mathbb{N}$. Define the function $r_\sigma(n,i)$ to be the number of atomic links of $\Delta_n$ categorized as the type $A_i^\sigma \times B^\sigma_{n-1-i}$. We find that the $f$-polynomial of every atomic link of type $A_i^\sigma \times B_{n-1-i}^\sigma$ is equal to the product of $f$-polynomials, $f^{A_i^\sigma}(s) \times f^{B_{n-1-i}^\sigma}(s)$. As a result, we find
%
%\[
%	R^{\Delta_n} (s) = \sum_{\sigma \in S} \sum_{i=0}^{n-1} r_\sigma(n,i) f^{A_i^\sigma}(s) \times f^{B_{n-1-i}^\sigma}(s) .
%\]
%
%
%
%
%
%%Consider the case where $\Delta_0,\Delta_1, \ldots$ is a sequence of simplicial complexes, and there is a set of simplicial complexes $A^\sigma_n, B^\sigma_n$ indexed by shape $\sigma \in S$ and $n \in \mathbb{N}$. Consider the case that every atomic link in $\Delta_n$ is isomorphic to the product of two simplicial complexes $A^\sigma_i \times B^\sigma_{n-1-i}$. Furthermore, the $f$-polynomial of $A^\sigma_i \times B^\sigma_{n-1-i}$ is $f^{A^\sigma_i}(s) \times f^{B^\sigma_{n-1-i}}(s)$. If we can enumerate that for $\Delta_n$, there are $r_\sigma(n,i)$ atomic links of type $A^\sigma_i \times B^\sigma_{n-1-i}$, we find that the bivariate atomic link sum polynomial is equal to
%%
%%\[
%%	\sum_{\sigma \in S} \sum_{i=0}^{n-1} r_\sigma(n,i) f^{A^\sigma_i}(s) \times f^{B^\sigma_{n-1-i}}(s) t^n
%%\]
%
% If $r_\sigma$ is separable to $r_\sigma^A(i) \cdot r_\sigma^B(n-1-i)$, this can be rewritten as the product
%
%\[
%	\sum_{\sigma \in S} t \left( \sum_{n\ge 0} r_\sigma^A(n) f^{A^\sigma_n} (s) t^n\right)
%\left( \sum_{n\ge 0} r_\sigma^B(n) f^{B^\sigma_n} (s) t^n\right) .
%\]
%
%Viewing each part of this product as a power series in $t$, we see the map taking power series $\sum_{n \ge 0} f^{A^\sigma_n}(s)t^n$ to power series $\sum_{n\ge 0} r_\sigma^A(n) f^{A^\sigma_n}(s) t^n$ is a \emph{linear operator} in $t$ on the set of formal power series on $\R[s]$. Write this linear operator as $O_t^{A^\sigma}$, and define $O_t^{B^\sigma}$ in a similar manner. We know that every linear operator on $t$ can be rewritten in the form $\sum_{n \ge 0} \mathfrak{M}(p_n) D_t^n$, where $\mathfrak{M}(p_n)$ is the linear operator representing multiplication by a polynomial $p_n$. \danger{I read this for polynomials, but it might only be true for polynomials and not power series... we might say that for all of the example cases used in this paper, the linear operators found have been of this form.} This expression can now be simplified as follows.
%
%%\begin{theorem}
%%A linear operator on the ring of formal power series on $\R[x]$ is an endomorphism on the ring of formal power series, and can be written as a sum $\sum_{n \ge 0} \mathfrak{m}(p_n) D_x^n$, where $\mathfrak{m}(p_\alpha)$ is the operator representing multiplication by the polynomial $p_\alpha$, and $D_x$ is the differential operator on $x$. \danger{Am I thinking of just finite operators? eesh...}
%%\end{theorem}
%%
%%Note that when 
%%
%%\danger{Let's write the operators $O^{A^\sigma}_t [f^{A^\sigma}(s)] = \sum_{n \ge 0} r_\sigma^A(n) f^{A^\sigma_i}(s) t^n$. It is an operator on $f^{A^\sigma_i}$.}
%
%\[
%	D_s f^{\Delta} (s,t) = \sum_{\sigma \in S} t O^{A^\sigma}_t\left[f^{A^\sigma}(s,t)\right] O_{t}^{B^\sigma} \left[f^{B^\sigma}(s,t)\right]
%\]
%
%We can rewrite a dual expression of this equation for the case where each simplicial complex belonging to a family $\Delta, A^\sigma, B^\sigma$ is polyhedral. We note that in this case, for each shape $\sigma$, there will be $r_\sigma(n,i)$ facets of $P(\Delta_n)$ of type $P(A_i^\sigma) \times P(B_{n-1-i}^\sigma)$. For a sequence $\{\Delta_0,\Delta_1, \ldots\}$ of simplicial complexes dual to simple polyhedra $\{P(\Delta_0), P(\Delta_1), \ldots\}$ with each polyhedron $P(\Delta_n)$ being $n$-dimensional, we know from the duality of bivariate $f$-polynomials that $f^{\Delta}(s,t)=f^{P(\Delta)}(x,y)$ when $x=1/s$ and $y=st$. This will allow us to make a statement about the bivariate generating function for the family of polyhedra $P(\Delta)$. Replacing some of the terms gives
%
%\[
%	D_s f^\Delta(s,t) = \sum_{\sigma \in S} xy \left(r^A_\sigma(n) f^{P(A^\sigma_n)}(x)y^n\right)
%	\left(r^B_\sigma(n) f^{P(B^\sigma_n)}(x)y^n\right).
%\]
%
%Application of the chain rule finds that $D_s f^\Delta(s,t) = xy D_y f^{P(\Delta)}(x,y) - x^2 D_x f^{P(\Delta)}(x,y)$. Using this, we can rewrite both sides of this equation and simplify by dividing by $x$. Now, note that $O^{A^\sigma}_t$ and $O^{B^\sigma}_t$ are both determined by the form of $r^A_\sigma$ and $r^B_\sigma$, expressed as operations on generating functions. Because this new equation has the same form, we find we can rewrite this equation by using operators $O^{A^\sigma}_y$ and $O^{B^\sigma}_y$, obtained by switching the variable but not the form of each operator. Rewriting the equation in this way gives us the new differential equation relating bivariate $f$-polynomials of polyhedra.
%
%\[
%	yD_y f^{P(\Delta)}(x,y)-x D_x f^{P(\Delta)}(x,y) = \sum_{\sigma \in S} y O^{A^\sigma}_y \left[f^{P(A^\sigma)}(x,y)\right]O^{B^\sigma}_y\left[f^{P(B^\sigma)}(x,y)\right]
%\]
%
%%Note that the operators $O^{A^\sigma}_y$ and $O^{A^\sigma}_t$ in this case are identical, save the change of variable from $y$ to $t$, making conversion between these two differential equations trivial. 
%
%\subsubsection{$\p$-graph case}
%
%Consider the case where $Q_0, Q_1, \ldots$ is a family of simple polyhedra, with each $Q_n$ being $n$-dimensional, and $G_0, G_1, \ldots$ is a series of graphs such that each $G_n$ is a $Q_n$-graph. Write $\nest{G_n}{Q_n}=P_n$. We know that every facet of $P_n$ is combinatorially isomorphic to the product of two $\p$-graph associahedra. Specifically, for a tube $t$ in $G_n$, we find the face $\Phi_t$ of $P_n$ is combinatorially isomorphic to the product of the $F_t$-graph associahedron of $G_n/t$, where $F_t$ is the face of $P_n$ associated with tube $t$, and the simplex-graph associahedron of $G_n|_t$. If the sets of possible $\p$-graphs of the form $G_n/t$ and $G_n|t$ are both easily iterated over, then this family of polyhedra is a good candidate for the atomic link/facet sum method. \danger{easily iterated over is so vague...}
%
%%This method is possible to apply when there exists an upper bound to the sizes of $\{G|_t : t \textrm{ is a tube of } G_n\}$ and $\{G / t: t \textrm{ is a tube of } G_n\}$ for all $n$. 
%
%Categorize all tubes of each graph $G_n$ into single-parameter families based on their induced graphs and reconnected complements, such that each graph $G|_t$ is in the family of simplex-graphs $A^\sigma$ and $G/t$ is in the family $B^\sigma$. We require that $A^\sigma_i$ is combinatorially isomorphic to an $i$-dimensional simplex-graph associahedron, and $B^\sigma_i$ is combinatorially isomorphic to an $n-1-i$-dimensional $\p$-graph associahedron.
%
%Note that here, we are defining $A$ and $B$ as the $\p$-graphs themselves, not the associated $\p$-graph associahedra. 
%
%We typically categorize two tubes $t, t'$ with the same number of vertices as having the same shape $\sigma$ if the graphs $G_n|_t$ and $G_n|_{t'}$ are isomorphic, and the $\p$-graphs $G_n/t$ and $G_n/t'$ are isomorphic.
%
%%Note that it is possible for $A^\sigma$ or $B^\sigma$ to represent the original family $G_0,G_1,\ldots$, or a family containing exactly one graph: the empty graph, for $A^\sigma_0$ or $B^\sigma_0$. We typically categorize two tubes $t, t'$ with the same number of vertices as having the same shape $\sigma$ if the graphs $G_n|_t$ and $G_n|_{t'}$ are isomorphic, and the $\p$-graphs $G_n/t$ and $G_n/t'$ are isomorphic.
%
%
%
%%In this case, we say that a tube $t \in G$ has \emph{shape $\sigma$} if the simplex-associahedron of $t$ is isomorphic to a polyhedron in the family $A^\sigma$, and 
%
%%We wish to derive a differential equation for bivariate polynomials $f^P$ and $f^{\Delta(P)}$. We note that facets of $P$-graph associahedra are each dual to individual tubes in the graphic tubing complex of the defining graph, and are combinatorially isomorphic to products of $\p$-graph associahedra and simplex-graph associahedra.
%
%For each $n$, we categorize all possible tubes of $G_n$ according to \emph{shape}, defining families of polyhedra of the form $A^\sigma, B^\sigma$ for each shape $\sigma$, such that for a tube $t$ of shape $\sigma$, the simplex-associahedron of $G|_t$ is a polyhedron isomorphic to a member of the family $A^\sigma$, and the $\p$-associahedron of the reconnected complement of $t$ is a polyhedron isomorphic to a polyhedron in the family $B^\sigma$. We find then that if $t$ contains $i+1$ vertices, then the induced simplex-graph associahedron of $G|_t$ is $i$-dimensional, and the $\p$-graph associahedron of $G/t$ is $n-1-i$-dimensional.
%
%Next we define a function $r_\sigma(n,i)$ for each shape $\sigma$ which enumerates the number of tubes of shape $\sigma$ and size $i+1$ in $G_n$. These are then sufficient to write a differential equation for the bivariate $f$-polynomials of the nested complexes of $G$ and the $\p$-graph associahedra of $G$.
%
%\danger{In this paper, we are primarily interested in the bivariate $f$-polynomials of graph associahedra. For a family $A$ of $\p$-graphs $A_0, A_1, \ldots$, we will write $f^{A}(x,y)$ as the bivariate $f$-polynomial of the graph associahedra of $A$, and write $A(n,k)$ as the term $f^{\Delta(A)}_{n,k}$ of the bivariate $f$-polynomial $f^{\Delta(A)}(s,t)$ of the tubing complexes of $A$, or the number of tubings of $A_n$ containing $k$ tubes.}
%
%
%
%%\subsection{Example: Associahedra}
%%
%%
%%
%%Say that $\{P_n|n \ge 0\}$ is the family of $n$-dimensional associahedra, defined here as path-associahedra. We wish to enumerate the $f$-vector of each $P_n$. Whether we choose to use the $f$-vectors of the polyhedra or their dual simplicial complexes, this starts by listing all possible facet or atomic link shapes, and counting $r_\sigma(n,i)$ for each shape $\sigma$. In this case, $P_n$ is the graph associahedron of the path on $n+1$ vertices. All tubes are paths in this graph, as are the reconnected complements, so we find that every facet of this graph associahedron is equal to the Cartesian product of a path on $i+1$ vertices, and a path on $n-i$ vertices. For each $0 \le i \le n-1$, there are $(n+1-i)$ tubes in the path containing $i+1$ vertices. As a result, we may say that there are $r_\sigma(n,i) = (n-1-i)$ facets of type $P_i \times P_{n-1-i}$.
%%
%%This formula gives us
%%
%%\[
%%	(yD_y - xD_x) f^P(x,y) = \sum_{n \ge 1}^\infty  y \sum_{i=0}^{n-1} (n-1-i+2) \left(f_{i}^{P}(x)y^i \right) \left(f_{n-1-i}^{P} (x) y^{n-1-i}\right).
%%\]
%%
%%Note that $r_\sigma(n,i)$ is separable in terms of $i$ and $n-1-i$, giving $r_\sigma^A(j)=1$ and $r_\sigma^B(j)=j+2$. From this, we see that $O_y^{A_\sigma}$ is the identity operator, and $O_y^{B^\sigma}=(yD_y+2)$. This becomes the partial differential equation
%%
%%\[
%%	(yD_y-xD_x) f^P(x,y) = y f^P(x,y) \left[y D_y f^P(x,y) + 2 f^P(x,y)\right].
%%\]
%%
%%This can be checked against the known bivariate $f$-polynomial for associahedra,
%%
%%\[
%%	f^P(x,y) = -\frac{\sqrt{x^2 y^2-2 (x+2) y+1}+(x+2) y-1}{2 (x+1) y^2},
%%\]
%%
%%which we find is indeed a solution. If we wish to find the bivariate $f$-polynomial of the dual simplicial complexes of $P_0, \ldots$, this becomes the differential equation
%%
%%\[
%%	D_s f^{\Delta}(s,t) = t (f^\Delta(s,t)) \left[t D_t f^\Delta(s,t) + 2 f^\Delta(s,t)\right]
%%\]
%%
%%which has as a solution
%%
%%\[
%%	f^{\Delta(P)}(s,t) = -\frac{\sqrt{t^2-2 (1+2s)t+1}+(1+2s) t-1}{2 (1+s) st^2}.
%%\]
%%
%%%\section{Grand theory of half open polyhedra and links}
%%%
%%%Taking a sub-face of a simple polyhedron is equivalent to taking a link of its dual simplicial complex, but in some cases we will find that operations on simplicial complexes do not generalize to 
%%%
%%%\begin{definition}
%%%A \emph{half-open polyhedron} is any convex collection of points in a vector space $\R^n$ defined by a finite set of inequalities $\{cx \le a\}$ and a finite set of strict inequalities $\{dx < b\}$.
%%%\end{definition}
%%%
%%%\begin{proposition}
%%%For any polyhedron $P$ and a set of proper faces $F_1,\ldots, F_k$ of $P$, the set $P \backslash (F_1 \cup F_2 \cup \cdots \cup F_k)$ is a half-open polyhedron. Call this a \emph{shaving} of $P$.
%%%\end{proposition}
%%%
%%%Every half-open polyhedron $Q$ is equal to a shaving of its \emph{closure} $\overline{Q}$.
%%%
%%%\begin{definition}
%%%A \emph{face} of a half-open polyhedron $Q$ is any set of points $F$ such that there exists a linear inequality $cx \le b$ for all $x \in Q$ and $x \in F$ if and only if $cx=b$ and $x\in Q$.
%%%\end{definition}
%%%
%%%This is exactly the definition of faces for polyhedra, but note that if $Q$ is a shaving of $P$ by a set of faces $\mathcal{F}$, any face $F \in \mathcal{F}$ or any of its subfaces is not a face of $Q$.
%%%
%%%\begin{definition}
%%%Two half-open polyhedra are \emph{combinatorially isomorphic} if their face posets are isomorphic.
%%%\end{definition}
%%%
%%%Note that their closures are not necessarily isomorphic.
%%%
%%%\begin{example}
%%%In the case of a $1$-simplex, shave off one vertex. The resulting half-open polyhedron is combinatorially isomorphic to a ray.
%%%\end{example}
%%%
%%%Note that not all half-open polyhedra are combinatorially isomorphic to polyhedra.
%%%
%%%\begin{example}
%%%The shaving of a $2$-simplex by all its vertices is not combinatorially isomorphic to any polyhedron.
%%%\end{example}



\section{Maximal tube sub-complexes for enumerating $f$-polynomials} \label{sec:method-two}

The previous section relies upon a method of overcounting, where faces of simplicial complexes or simple polyhedra are counted more than once and our count is adjusted accordingly. This section presents a method where tubings are divided by cases, and each tubing is counted exactly once. The broad concept is as follows: for any tube $t$, we wish to characterize all tubings $T$ that contain the tube $t$, such that $t$ is maximal in $T$. Next, we wish to pick a set of tubes $t_1, \ldots, t_k$ such that only one tube out of the set can ever be maximal in a tubing at the same time. Finally, we characterize the set of tubings that do not contain any tube in the set $t_1, \ldots, t_k$.
%
%
%\danger{I really do not like this following example enumeration. It may make more sense to just get rid of it.}
%
%\subsection{Example enumeration}
%
%Consider the path graph on the five elements of the set $[5]$ as a simplex-graph. For every possible tubing $T$, we will ask the question: what is the largest tube $t \in T$ which contains the vertex $1$? We find that either $t=[1]$, $[2]$, $[3]$, or $[4]$, or $1$ is not in any tube in $T$. Figure \ref{fig:path-graph-maximal-tubings} illustrates these five possibilities. We note that if $t=[k]$, then the vertex $k+1$ cannot be in $T$.
%
%Now we wish to enumerate the number of tubings $T$ such that the tube $t=[k]$ for $1 \le k \le 4$ is maximal in $T$; we can call this the maximal tube sub-complex of $t$. We note that for each tubing $T$ in the maximal tube sub-complex of $t$, $T \backslash t$ consists of a tubing on the path graph from $1$ to $k$ not containing $[k]$, and a tubing on the path graph from $k+2$ to $5$. When $k=2$, we note there are $3$ possible tubings of the path graph on $[2]$, and $6$ possible tubings of the vertices $\{4,5\}$, and so there are $18$ possible tubings containing $[2]$ as a maximal tube.
%
%%We find that there are three possibilities: either $t=\{1\}, t=\{1,2\}, t=\{1,2,3\}$, or no tube $t \in T$ contains $1$. Figure \ref{fig:path-graph-maximal-tubings} illustrates these four possibilities. We also note that when $t=\{1\}$, no tube in $T$ can contain the vertex $2$; when $t=\{1,2\}$, no tube in $T$ can contain $3$; and when $t=\{1,2,3\}$, no tube in $T$ can contain $4$. We then see in the figure red crosses to indicate vertices which cannot be contained in any such tubing. However, we note in this case that the remaining vertices are divided into two path graphs.
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=.5\textwidth]{Chapter-3/figs/path-graph-maximal-tubings.pdf}
%\caption{A categorization of possible maximal tubes containing the vertex $1$ in a path simplex-graph.} \label{fig:path-graph-maximal-tubings}
%\end{figure}
%
%This is an example of enumerating tubings in the maximal tube sub-complex of the tube $t=\{1,2\}$. We would be able to finish enumeration by counting the number of tubings in the maximal tube sub-complexes for each case.
%
%This illustrates the general method of maximal tube sub-complex enumeration. In general, we will describe a set of tubes such that the maximal tube sub-complexes of these tubes covers the entire tubing complex of a graph. Then, we will decompose each maximal tube sub-complex as the product of an induced graph tubing complex, and the graph tubing complex of the \emph{neighborless complement} of a tube. Finally, we will use the atomic link sum polynomial method of writing an equation involving counting functions of the form $r_\sigma$, and this will yield a result equivalent to Proposition \ref{prop:diff-eq}.
%
%
%Similar to the method of atomic link sum enumeration, for each graph of dimension $n$ we will be counting the number of tubings with $k$ tubes.
%
%%The goal of this method is to enumerate all $k$-element tubings of a $\Delta$-graph by dividing all tubings into cases, and counting each tubing exactly once. We will do this by counting tubings such that a certain tube is maximal.
%
%%As an example, consider the associahedron. It is a simplex-graph associahedron, whose graph is a path on $n+1$ vertices. Consider a tubing $T$. Either no tube $t$ in $T$ contains the vertex $1$, or there is at least one tube such that $1 \in t \in T$. All tubes containing $1$ are of the form $[i+1]=\{1,2,\ldots,i+1\}$ for $0 \le i \le n-1$, and if $1$ is in a tube in $T$, then there exists a unique tube $[i+1]$ which is in $T$ and which is maximal in $T$.
%%
%%Now it is clear that every tubing $T$ falls into a unique case. Either $[i+1] \in T$ for some $0 \le i \le n-1$ and $[i+1]$ is maximal in $T$, or $1$ is not in any tube in $T$. The former cases are easy to count; the remaining tubes must be sub-tubes of $[i+1]$, or subsets of the vertex set $\{i+3,i+4,\ldots,n+1\}$. The latter case is also easy to count, as this tubing must be a $k$-tubing on a path graph on $n$ vertices.
%
%%This section formalizes the concept of counting subcomplexes where a tube $t$ is maximal. It gives tools to allow a more generalized version of the associahedron enumeration outlined here. 
%
%%	For a simplicial complex $\Delta$ on base set $\mathcal{S}$, for a subset $X \subset \mathcal{S}$ we can define the \emph{elimination} of $X$ in $\Delta$ as the simplicial complex on $\mathcal{S}\backslash X$ such that, for each $F \in \Delta$, we find $F \in \Delta\backslash X$ if $F \cap X = \emptyset$.
%
%% Together with the link operation, $\Delta/X$ and $\Delta\backslash X$ are two of the most basic operations on simplicial complexes. We note that $f^\Delta(s) = s^{|X|} f^{\Delta/X}(s) + f^{\Delta\backslash X}(s)$ for any pair $X \in \Delta$. We can create further partitions of $\Delta$ using further link and elimination operations.
%
%%	We have been able to define $N(G,\Delta)/\{t\}$ for some tube $t$ in terms of a nested complex on $\Delta/t$, which is itself a simplicial complex. It is our attempt now to define 
%
%%	When $\Delta$ is the tubing complex of a $\p$-graph, we can calculate $\Delta/T$ as a product of a $\p$-graph tubing complex and simplex-graph tubing complexes through a process of reconnected complements. However, $\Delta\backslash T$ 
%
%%	\subsubsection{Element deletion operation}
%%
%%	\danger{Here I am using notation $N(\Delta, G)$...}
%%
%%		For a simplicial complex $\Delta$ on base set $\mathcal{S}$, $\Delta$-graph $G$, and vertex set $X \subseteq \mathcal{S}$, the graph $G \backslash X$ is the graph on vertex set $\mathcal{S} \backslash X$. We can define a new nested complex, $N(\Delta\backslash X, G \backslash X)$.
%%
%%		\begin{proposition}
%%			The nested complex $N(\Delta\backslash X, G \backslash X)$ is equal to $N(\Delta,G) \backslash \danger{intset}_X$, where $intset_X$ is the set of $\Delta$-tubes of $G$ which intersect with $X$. \danger{I made up intset on the fly, but it's the intersection set...}
%%		\end{proposition}

	\subsection{Maximal tube sub-complexes}

\newcommand{\nestmax}[3]{\mathcal{N}_{/#3 \max}(#1, #2)} % commands {G}{\Delta}{t}


		\begin{definition}
		The maximal tube sub-complex $\nestmax{G}{\Delta}{t}$ is the set of all tubings such that $t \notin T$, $\{t\} \cup T$ is a valid tubing and $t$ is maximal in $\{t\} \cup T$.
	\end{definition}

	This is equivalent to taking the set of tubings $T$ such that $t \in T$ and $t$ is maximal in $T$, and removing $t$ from $T$. It is also equivalent to taking the complex $\mathcal{N}(G,\Delta)$, removing any tubes which contain $t$ as a proper subset, and then taking the link of $t$ in this new complex.

	Define $n(t)$ to be the \emph{neighborhood} of a tube $t$ in $G$; that is, if $v \in t$ or $v$ is adjacent to a vertex in $t$, then $v \in n(t)$. Define $xn(t) = n(t) \backslash t$ to be the \emph{exclusive neighborhood} of $t$. For a graph $G$ and vertex subset $S$, we define the graph $G \backslash S$ to be just the graph induced on the complement of $S$ in the vertex set of $G$. For a simplicial complex $\Delta$ and subset $S$ of the base set of $\Delta$, we define $\Delta \backslash S$ to be the simplicial complex obtained by deleting any faces containing any elements of $S$.

	\begin{proposition} \label{prop:deleted-vertices-in-graph-stuff}
		The tubing complex $\mathcal{N}(G/S,\Delta/S)$ for any subset $S$ of the base set of $\Delta$ is equal to the set of tubings in the complex $\mathcal{N}(G,\Delta)$ such that $t \cap S = \emptyset$ for each tube $t$ in the tubing.
	\end{proposition}

	

	\begin{definition}
		The \emph{neighborless complement} of a tube $t$ in a $\Delta$-graph $G$ is the $(\Delta/t)\backslash xn(t)$-graph $(G/t) \backslash xn(t)$.
	\end{definition}

	We can now prove a statement:

	\begin{proposition}
		For a graph $G$ with tube $t$, the tubing complex $\mathcal{N}((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$ of the neighborless complex is equal to the set of tubings $T$ in $\nestmax{G}{\Delta}{t}$ such that, for every tube $t' \in T$, $t' \cap t = \emptyset$.
	\end{proposition}

	\begin{proof}
	We wish to characterize the tubes in $\nestmax{G}{\Delta}{t}$. This complex contains all tubes $t' \subset t$, which are tubes of the simplex-graph $G|_t$. It also contains all tubes $t'$ such that $t, t'$ are compatible and $t' \not\subseteq t$ and $t \not\subseteq t'$. We note that if $t, t'$ are compatible, then $t \subset t'$ if and only if $t' \cap xn(t) = \emptyset$. Recall also that $t'$ is a tube compatible with but not contained in $t$ if and only if $t' \backslash t$ is a tube of $G/t$. As a result, we note that for two compatible tubes $t, t'$, we find $t \not\subseteq t', t' \not\subseteq t$ if and only if $t'$ is a tube of $G/t$ not containing any vertex in $xn(t)$. 
	
	Now we note that $T$ is a tubing in $\nestmax{G}{\Delta}{t}$ if and only if it is a tubing in $G/t$ containing no vertex in $xn(t)$ in any of its tubes. Proposition \ref{prop:deleted-vertices-in-graph-stuff} shows that this is the case if and only if $T$ is a tubing of $(G/t)\backslash xn(t)$.
\end{proof}



	Figure \ref{fig:neighborless-complement} illustrates the finding of the neighborless compelement of a tube in a hypercube-graph in three steps. First, we take the reconnected complement; this removes the vertices in $t$ from $G$, as well as any vertices not in $\Delta/t$, which in this case is the vertices of $-t$. Finally, we remove all neighbors of $t$.

\begin{figure}
\centering
\includegraphics[width=.5\textwidth]{Chapter-3/figs/neighborless-complement}
\caption{Reconnected complement and neighborless complement of a tube in a hypercube graph.}\label{fig:neighborless-complement}
\end{figure}

\danger{The nested complex notation says $\mathcal{N}(\B,\Delta)$, so $\mathcal{N}(G, \Delta|t\max )$ might be the correct version. Maybe even $\mathcal{N}(G,\Delta,t=\max)$ ?? One problem is that I have $G|_t$. So maybe $\mathcal{N}_{t\max}(G,\Delta)$. I am converting this to a newcommand to make things easier on me.}




	%This complex is equal to the link of $\{t\}$ in $N(G,\Delta)$, minus any tubes which contain $t$ as a subset. Note though that in the standard isomorphism between tubes in $G$ which are not subsets of $t$ and tubes in the reconnected complement $G/t$, a tube $s$ in the reconnected corresponds to a tube $s \cup t$ containing $t$ as a subset if and only if $s$ contains a vertex in the neighborhood of $t$. As a result, the tubing complex 

	For a graph $G$, refer to $\mathcal{N}(G)$ as the simplex-graph tubing complex of $G$. We can now characterize maximal tubing complexes entirely.

	\begin{proposition}
		The complex $\nestmax{G}{\Delta}{t}$ is equal to the Cartesian product of tubing complexes $\mathcal{N}(G|_t)$ and $\mathcal{N}((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$.
	\end{proposition}

	\begin{proof}

	We know that the set of tubes $t'$ in the base set of $\nestmax{G}{\Delta}{t}$ such that $t' \cap t=\emptyset$ are just tubes of the neighborless complement of $t$. The tubes $t'$ in $\nestmax{G}{\Delta}{t}$ such that $t' \cap t \ne \emptyset$ are exactly the tubes which are subsets of $t$, and all such proper subsets are tubes of the simplex-graph $G|_t$. We then note that any tube $t'$ in the neighborless complement and any tube $t''$ in $G|_t$ are disjoint and non-adjacent, and so it is trivial to see that every tubing $T$ is equal to the disjoint union of a tubing in the neighborless complement of $t$ and $G|_t$, and the maximal tube complex of $t$ is equal to the product of the two complexes.

%	We wish to first characterize the tubes in $\nestmax{G}{\Delta}{t}$. This complex contains all tubes $t' \subsetneq t$, which are tubes of the simplex-graph $G|_t$. It also contains all tubes $t'$ such that $t, t'$ are compatible and $t' \not\subseteq t$ and $t \not\subseteq t'$. We note that if $t, t'$ are compatible, then $t \subsetneq t'$ if and only if $t' \cap xn(t) = \emptyset$. Recall also that $t'$ is a tube compatible with but not contained in $t$ if and only if $t' \backslash t$ is a tube of $G/t$. As a result, we note that $t, t'$ are compatible, with $t \not\subseteq t'$ and $t' \not\subseteq t$, if and only if $t'$ is a tube of $G/t$ not containing any vertex in $xn(t)$. This is then equivalent to saying that $t'$ is a tube of the $(\Delta/t)\backslash xn(t)$-graph $(G/t)\backslash xn(t)$.
%
%	As a result, the set of tubes in $\nestmax{G}{\Delta}{t}$ is equal to the disjoint union of the tubes in $\mathcal{N}(G|_t)$ and the tubes in the neighborless complement of $t$. We then note that because the vertex sets of the two graphs are disjoint and non-adjacent, any tubing of one graph is compatible with a tubing of the other graph, and we can see that the complex $\nestmax{G}{\Delta}{t}$ is isomorphic to the Cartesian product of the other two tubing complexes.
	\end{proof}

%	\begin{proof}
%			The complex $\nestmax{G}{\Delta}{t}$ is equal to the link of $\{t\}$ in $\mathcal{N}(G,\Delta)$, minus any tubes which contain $t$ as a subset. We will first prove that the base set of $\nestmax{G}{\Delta}{t}$ is equal to the disjoint union of the set of simplex-tubes of $G|_t$, and the base set of $\mathcal{N}((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$. Then, it will be trivial to see that the two complexes are equal.
%
%			Propositions \ref{prop:pseudolink-graph} and \ref{prop:singletonlink} together show the link of $\{t\}$ is isomorphic to the product of $\mathcal{N}(G/t,\Delta/t)$ and the simplex-nested complex on $G|_t$, with the map taking $s$ to the tube $s \in G|_t$ if $s \subsetneq t$, and taking $s$ to $s \backslash t$ if $s \not\subseteq t$.
%
%			We now note that for a tube $s$ in the link of $t$ such that $s \not\subseteq t$ that $s \ne s\backslash t$ if and only if $t \subsetneq s$. We then note that for connected subgraphs, $t \subsetneq s$ implies that $s \cap xn(t) \ne \emptyset$. Now for tubes, we find $s \cap xn(t) \ne \emptyset$ and $\{s,t\}$ are compatible if and only if $t \subsetneq s$. As a result, for each tube $s$ in the link of $t$ in $G$, $t \not\subseteq s$ if and only if $xn(t) \cap s \ne \emptyset$. In addition, if $s'$ is a tube in the reconnected complement of $G$ and $s' \cap xn(t) = \emptyset$, then $s'$ is in the link of $t$ in $G$ and $t \cap s' = \emptyset$. As a result, we find that the base set of $\nestmax{G}{\Delta}{t}$ is equal to the union of the tube sets of $G|_t$ and $(G/t)\backslash xn(t)$. It is then trivial to see that every tubing in $\nestmax{G}{\Delta}{t}$ is equal to the union of a tubing of the simplex-graph $G|_t$ and a tubing in $\mathcal{N}((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$, and showing that each union of two such tubings defines a tubing in $\nestmax{G}{\Delta}{t}$ proves that $\nestmax{G}{\Delta}{t}$ is equal to the Cartesian product of the two.		
%	\end{proof}

	Now that we have defined the maximal tube complex of a tube $t$, we need to find an easy method to characterize a set of tubes such that no two tubes in the set can ever both be maximal. We also wish to be able to easily enumerate the set of tubings which contain no tubes in $T$.

	Consider a $\Delta$-graph $G$. For a set $X$ of vertices of $G$, define $intset_X$ to be the set of tubes of $G$ that have nonempty intersection with $X$. We define a \emph{kingmaker set} to be a set $X$ of vertices of a $\Delta$-graph $G$ such that, for any two compatible tubes $t_1, t_2 \in intset_X$, we find $t_1 \subset t_2$ or $t_2 \subset t_1$. There are several ways this condition may hold; for instance, every clique in a graph is a kingmaker set, even including every 1-clique.

	We note that for every tubing $T$ of a graph with kingmaker set $X$, either there exists a unique tube $t \in intset_{X}$ such that $t \in T$ and $t$ is maximal in $T$, or no tube in $T$ intersects with $X$. In the first case, $T \backslash \{t\}$ is in $\nestmax{G}{\Delta}{t}$. In the second case, $T \in \mathcal{N}(G\backslash X, \Delta\backslash X)$. We recall that $f^{\mathcal{N}(G,\Delta)}(s)=\sum_{k\ge 0} f_k s^k$ counts the number of tubings of size $k$ in $G$. As a result, the $f$-vector of the set of tubings such that $t$ is maximal is equal to $s$ times the $f$-vector of $\nestmax{G}{\Delta}{t}$, giving us the following equation.

	\begin{proposition} \label{prop:kingmaker-partition}
		For a $\Delta$-graph $G$ with kingmaker set $X$,
		\[
			f^{\mathcal{N}(G,\Delta)} (s) = f^{\mathcal{N}(G\backslash X, \Delta \backslash X)} + s \sum_{t \in intset_X} f^{\nestmax{G}{\Delta}{t}}(s)
			.
		\]
	\end{proposition}

	Finally, we recall that we can write $\nestmax{G}{\Delta}{t}$ as a Cartesian product of tubing complexes. If $\mathcal{N}(G|_t)$ is the simplex-graph tubing complex induced by $G|_t$, we get the following equation.

	\begin{proposition} \label{prop:kingmaker-partition-2}
		For a $\Delta$-graph $G$ with kingmaker set $X$,
		\[
			f^{\mathcal{N}(G,\Delta)} (s) = f^{\mathcal{N}(G\backslash X, \Delta \backslash X)} + s \sum_{t \in intset_X} 
	f^{\mathcal{N}(G|_t)}(s)
	f^{\mathcal{N}((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))}(s).
		\]
	\end{proposition}

	\begin{remark}
		What is the rank of $\mathcal{N}(G\backslash X, \Delta\backslash X)$ or $\nestmax{G}{\Delta}{t}$? We recall that if $\Delta$ is a pure simplicial complex of rank $n$ with face $S$, then $\Delta/S$ is rank $n-|S|$, allowing us to very nicely index our terms and create a function of bivariate generating polynomials. In contrast, if $X$ is a set in the base set of $\Delta$, then $\Delta \backslash X$ could have any rank between $n-|X|$ and $n$. We know the rank of $\mathcal{N}(G|_t)$ is $(|t|-1)$, and if $\Delta$ is a pure rank $n$ simplicial complex, then $(\Delta/t)$ is rank $(n-|t|)$. The rank of $(\Delta/t)\backslash xn(t)$ is then not fixed, and depends on the vertices in $xn(t)$.
	\end{remark}

	\subsection{Calculating $f$-polynomial through maximal tube enumeration}

	In this subsection, we will apply Proposition \ref{prop:kingmaker-partition-2} in order to calculate the bivariate $f$-polynomial of a family of $\Delta$-graph nested complexes. Consider a family of simplicial complexes $\Delta=\{\Delta_0,\Delta_1,\ldots\}$, where each simplicial complex $\Delta_n$ has rank $n$. Consider a family of $\Delta$-graphs $\{G_0,G_1,\ldots\}$ such that each graph $G_n$ is a $\Delta_n$-graph.

	We first wish to calculate the $f$-polynomials of each nested complex $\mathcal{N}(\Delta_n,G_n)$. We will pick a kingmaker $X_n$ for each graph $G_n$.
We will define a family of simplicial complexes $A_n^\sigma, B_n^\sigma$, indexed by shape $\sigma \in S$ and $n \ge 0$ such that $A_n^\sigma, B_n^\sigma$ are each rank $n$, along with constant $\gamma_\sigma$ for each $\sigma$, as follows.
Note that for each tube $t \in intset_{X_n}$ with $i+1$ vertices, the complex $\nestmax{G}{\Delta}{t}$ is isomorphic to the product of complexes $\mathcal{N}(G|_t)$ and $\mathcal{N}((G_n/t)\backslash xn(t),(\Delta_n/t)\backslash xn(t)))$.
The complex $\mathcal{N}(G|_t)$ must be rank $i$. The complex $(\Delta_n/t)$ must be rank $n-1-i$. However, the complex $(\Delta_n/t) \backslash xn(t)$ may be lower dimension. We define families $A$ and $B$ indexed by shapes $\sigma \in S$ such that the complex $(\Delta_n/t)\backslash xn(t)$ is rank $n-1-i-\gamma_\sigma$ for each $\sigma$, and $\mathcal{N}(G|_t)$ is isomorphic to $A_i^\sigma$ and $\mathcal{N}((G_n/t)\backslash xn(t),(\Delta_n/t)\backslash xn(t)))$ is isomorphic to $B_{n-1-i-\gamma_\sigma}^\sigma$ for each tube $t$ of shape $\sigma$ with $i+1$ vertices.	Finally, assume that the simplicial complex $\Delta_n \backslash X$ is rank $n-\rho$ for each $n \ge \rho$; we define a family $\{C_0,C_1,\ldots\}$ of simplicial complexes such that each $C_n$ is rank $n$ and $C_{n-\rho} = \mathcal{N}(G_n\backslash X_n, \Delta \backslash X_n)$. As a result, if $r_\sigma(n,i)$ is the number of tubes of shape $\sigma$ containing $i+1$ vertices, we find the following result:
	\[
		f^{\mathcal{N}(G_n,\Delta_n)} (s) = f^{C_{n-\rho}}(s) + s\sum_{\sigma \in S}
		\sum_{i=0}^{n-1-\gamma_\sigma}
		r_\sigma(n,i)
		f^{A^\sigma_i} (s)
		f^{B^\sigma_{n-1-\gamma_\sigma-i}}(s).
	\]

	We can then create a bivariate generating function by multiplying by $t^n$ and summing for each $n \ge \rho$.

	\danger{Using begin multiline gives me some real serious errors for some reason. environment multiline undefined, etc. So I am using align* which I think works well enough.}

		\begin{align*}
		\sum_{n \ge \rho} f^{\mathcal{N}(G_n,\Delta_n)} (s)t^n =& 
		\sum_{n \ge \rho} f^{C_{n-\rho}}(s)t^\rho +\\
		&\sum_{n \ge \rho} s\sum_{\sigma \in S}t^{1+\gamma_\sigma}
		\sum_{i=0}^{n-1-\gamma_\sigma}
		r_\sigma(n,i)
		f^{A^\sigma_i} (s)
		f^{B^\sigma_{n-1-\gamma_\sigma-i}}(s)
		t^{n-1-\gamma_\sigma}
	\end{align*}


%	\begin{lemma}
%		For any 
%	\end{lemma}
%
%	\bigskip
%
%
%For each $n$, we will choose a set $X_n$, a subset of the vertex subset of $G_n$, such that for any two strongly compatible tubes $t_1, t_2$ which intersect with $X_n$, we find $t_1 \subset t_2$ or $t_2 \subset t_1$. Any clique in $G_n$ satisfies this condition, but the choice greatly impacts the counting. Define $intset_{X_n}$ of a $\Delta$-graph to be the set of tubes which intersect with $X_n$.
%
%	Note that for a tubing $T$ of $G_n$, either the set $intset_{X_n} \cap T$ must have a maximal element, or $intset_{X_n} \cap T=\emptyset$. As a result, we can partition $\mathcal{N}(\Delta_n,G_n)$ into copies of $\mathcal{N}(\Delta_n,G_n: t \max)$ for $t \in intset_{X_n}$, as well as the set $\mathcal{N}(\Delta_n\backslash X_n, G_n \backslash G_n)$.
%
%	We must rewrite these tubing complexes as products of simplicial complexes belonging to families defined by shapes. Sort the tubes in $intset_{X_n}$ into shapes $\sigma \in S$ such that, for each tube $t$ of $G_n$ and shape $\sigma$ and size $i+1$, the simplex-graph tubing complex of $G_n|_t$ is isomorphic to a simplicial complex $A^\sigma_i$, and the tubing complex $N((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$ is isomorphic to some simplicial complex $B^\sigma_{n-1-i-\gamma_\sigma}$. Note that we are interested in enumerating the number of tubings where $t$ is maximal, so we must include $t$ in counting every tubing where $t$ is maximal. As a result, we must multiply the product of generating functions by $s$ to find the generating function $s f^{A^\sigma_i}(s)f^{B^\sigma_{n-1-\gamma-i}}(s)$.
%
%Write the function $r_\sigma(n,i)$ to count the number of tubes of shape $\sigma$ of size $i+1$ in $intset_{X_n}$. We are using the variable $\gamma_\sigma$ to reflect the fact that $N((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$ is not always a rank $n-1-i$ simplicial complex; sometimes, removing the vertices $xn(t)$ lowers the rank of the complex. Now assume that $\mathcal{N}(\Delta_n\backslash X_n, G_n \backslash X_n)$ is a rank $n-\rho$ simplicial complex $C_{n-\rho}$, and empty if $n < \rho$. The generating function for $\mathcal{N}(\Delta_n,G_n)$ becomes
%
%	\[
%		f^{\mathcal{N}(\Delta_n,G_n)} (s) = f^{C_{n-\rho}}(s) + s\sum_{\sigma \in S}
%		\sum_{i=0}^{n-1-\gamma_\sigma}
%		r_\sigma(n,i)
%		f^{A^\sigma_i} (s)
%		f^{B^\sigma_{n-1-\gamma_\sigma-i}}(s)
%	\]
%
%	for all $n \ge \rho$. \danger{I need to go back and really figure out, is this correct? Doesn't something weird happen when $n < \rho$? I think I remember needing a $+1$ when working with polyhedra, but not needing them when working with simplicial complexes.}
%
%		\[
%		\sum_{n \ge \rho} f^{\mathcal{N}(\Delta_n,G_n)} (s)t^n = 
%		\sum_{n \ge \rho} f^{C_{n-\rho}}(s)t^\rho +\sum_{n \ge \rho} s\sum_{\sigma \in S}t^{1+\gamma_\sigma}
%		\sum_{i=0}^{n-1-\gamma_\sigma}
%		r_\sigma(n,i)
%		f^{A^\sigma_i} (s)
%		f^{B^\sigma_{n-1-\gamma_\sigma-i}}(s)
%		t^{n-1-\gamma_\sigma}
%	\]

	We want to rewrite this equation by summing for all $n$, not just $n \ge \rho$. We will introduce a pair of error terms. Define  \[\epsilon_L=\sum_{n=0}^{\rho-1} f^{\mathcal{N}(G_n,\Delta_n)} (s)t^n\] for the left hand side, and

		\[
		\epsilon_R =
		\sum_{n =0}^{\rho-1} f^{C_{n-\rho}}(s)t^\rho +
		\sum_{n =0}^{\rho-1} s\sum_{\sigma \in S}t^{1+\gamma_\sigma}
		\sum_{i=0}^{n-1-\gamma_\sigma}
		r_\sigma(n,i)
		f^{A^\sigma_i} (s)
		f^{B^\sigma_{n-1-\gamma_\sigma-i}}(s)
		t^{n-1-\gamma_\sigma}.
	\]

	We are now able to rewrite an earlier equation as

		\begin{align*}
		&\left(\sum_{n \ge 0} f^{\mathcal{N}(G_n,\Delta_n)} (s)t^n \right)-\epsilon_L=\\
		&\sum_{n \ge 0}\left( f^{C_{n-\rho}}(s)t^\rho +
		s\sum_{\sigma \in S}t^{1+\gamma_\sigma}
		\sum_{i=0}^{n-1-\gamma_\sigma}
		r_\sigma(n,i)
		f^{A^\sigma_i} (s)
		f^{B^\sigma_{n-1-\gamma_\sigma-i}}(s)
		t^{n-1-\gamma_\sigma}\right)
		-\epsilon_R
	\end{align*}

	We again rewrite $r_\sigma(n,i)$ as a sum of separable equations, $r_\sigma(n,i)=\sum_{j=1}^k r_\sigma^{A,j}(i) r_\sigma^{B,j}(n-1-i-\gamma_\sigma)$. With these two substitutions, we can write







	\[
		f^{\mathcal{N}(G,\Delta)} (s) -\epsilon_L=-\epsilon_R+ f^{C}(s)t^\rho +\]

		\[
		\sum_{n\ge 0}
		\sum_{\sigma \in S}
		\sum_{j=1}^k
		st^{1+\gamma_\sigma}
		\sum_{i=0}^{n-1-\gamma_\sigma}
		r_\sigma^{A,j}(i)
		f^{A^\sigma_i} (s)
		t^i
		r_\sigma^{B,j}(n-1-i-\gamma_\sigma)
		f^{B^\sigma_{n-1-\gamma-i}}(s)
		t^{n-1-i-\gamma_\sigma}.
	\]

	We can then rewrite this convolution as a product of power series. Using the same definition of the linear operator $\sum_{n\ge0} r_\sigma^{A,j}(n) a_nt^n=O_t^{A,\sigma,j}[a(t)]$, we get a sum of products of linear operations on $f^{A^\sigma}$ and $f^{B^\sigma}$, which we can rewrite as the equation in the following proposition..

	\begin{proposition} \label{prop:maximal-tube-enumeration-big-result}
	Consider the case where $\Delta=\{\Delta_0,\Delta_1,\ldots\}$ is a family of simplicial complexes with $\Delta_n$ rank $n$, and graph family $G=\{G_0,G_1,\ldots\}$ is such that $G_n$ is a $\Delta_n$-graph, and $X_n$ is a kingmaker set of $G_n$ decomposing each complex $\nestmax{G}{\Delta}{t}$, for $t \in intset_{X_n}$ of shape $\sigma$ with $|t|=i+1$, into the product of the simplex-graph tubing complex of $G|_t$ isomorphic to $A_i^{\sigma}$, and the neighborless complement graph tubing complex of $t$ isomorphic to $B_{n-1-\gamma_\sigma-i}$. We also find a family of complexes $C=\{C_0,C_1,\ldots\}$ such that $\mathcal{N}(G_n,\Delta_n)$ is isomorphic to $C_{n-\rho}$ for all $n \ge \rho$. In this case, we find the following equation:
	\[
		f^{\mathcal{N}(G,\Delta)}(s,t)-\epsilon_L+\epsilon_R
		=
		f^C(s,t)t^\rho +
		st\sum_{\sigma \in S} t^{\gamma_\sigma} \sum_{j=1}^k
		O_t^{A,\sigma,j}\left[f^{A^\sigma}(s,t)\right]
		O_t^{B,\sigma,j}\left[f^{B^\sigma}(s,t)\right].
	\]

	\end{proposition}

	We now finish by taking note of $\epsilon_L$ and $\epsilon_R$. When $\rho=0$, these are both empty sums, and $\epsilon_L=\epsilon_R=0$. When $\rho=1$, $\epsilon_L=f^{\mathcal{N}(\Delta_0,G_0)}(s)$, and because $\Delta_0$ is is a rank $0$ simplicial complex, its tubing complex must be the empty set, and $\epsilon_L=1$. In calculating $\epsilon_R$, we calculate the terms for $n=0$, but indices $n-\rho$ and $n-1-\gamma_\sigma-i$ are all less than zero, and so $\epsilon_R = 0$. The calculation of $\epsilon_L, \epsilon_R$ is more complicated when $\rho \ge 2$, but we do not need this case for this thesis and so we omit this case.

		\subsection{Half-Open Polyhedra}\label{sub:halfopen}

	Using this method to enumerate tubings of $\Delta$-graphs requires the calculation of the graphs $(G/t)\backslash xn(t)$ and $G\backslash X_n$, and the simplicial complexes $(\Delta_n/t)\backslash xn(t)$ and $\Delta_n\backslash X_n$ When $\Delta$ is the dual simplicial complex of a polyhedron, we know that $\Delta_n/t$ is also dual to a polyhedron. However, we have no guarantee that $(\Delta_n/t)\backslash xn(t)$ or $\Delta_n\backslash X_n$ is dual to a polyhedron. In general, if $P$ is a a simple polyhedron and $S$ is a set of facets of $P$, it is possible for $\Delta(P)\backslash S$ to not be dual to any polyhedron. We will define a new class of shapes related to polyhedra, called half-open polyhedra, in order to understand this.


	\begin{definition}
	A \emph{half-open polyhedron} is any collection of points in a vector space $\R^n$ defined by a finite set of inequalities $\{cx \le a\}$ and a finite set of strict inequalities $\{dx < b\}$.
	\end{definition}

	Every half-open polyhedron is convex, and half-open polyhedra are a class of shapes which include polyhedra. Define the \emph{shaving} of a polyhedron $P$ by a set of proper faces $F_1,\ldots, F_k$ to be the set $P \backslash (F_1 \cup F_2 \cup \cdots \cup F_k)$.

	\begin{proposition}
	For any polyhedron $P$ and set of proper faces $S=\{F_1,\ldots, F_k\}$, the shaving of $P$ by $S$ is a half-open polyhedron.
	\end{proposition}

	\begin{proof}
		For each face $F_i$, there exists a vector $c_i$ in the normal cone of $F_i$ such that $c_i \cdot x$ is maximized on $F_i$, with $c_i \cdot x = a_i$ for all $x \in F_i$. The shaving of $P$ by $S$ is the half-open polyhedron defined by all non-strict inequalities defining $P$, and adding strict inequalities $c_i \cdot x < a_i$ for all $1 \le i \le k$.
	\end{proof}

	We define faces of half-open polyhedra in the same way we define faces of polyhedra.

		\begin{definition}
	A \emph{face} of a half-open polyhedron $Q$ is any set of points $F$ such that there exists a linear inequality $cx \le b$ for all $x \in Q$ and $x \in F$ if and only if $cx=b$ and $x\in Q$.
	\end{definition}

	\begin{proposition}
		Every half-open polyhedron is the shaving of a polyhedron by some set of faces.
	\end{proposition}
\begin{proof}
Consider a set of inequalities defining a half-open polyhedron $Q$ of the form $\{cx \le a\}$ and $\{dx < b\}$. Now define $Q'$ as the polyhedron defined by replacing every strict inequality $\{dx < b\}$ with the inequality $dx \le b$. We see that $Q'$ is a shaving of $Q$.
\end{proof}

%	\begin{proof}
%		This is straightforward, as 
%%		A finite set of inequalities is minimal if omitting any inequality does not define the same half-open polyhedron.
%%
%% 		Consider the half-open polyhedron $Q$ defined by a minimal set of inequalities. Consider an inequality $\{dx < b\}$ in this set, and define $Q'$ to be the polyhedron defined by omitting this inequality. Because $Q \ne Q'$, there must be points $x \in Q' \backslash Q$, such that $dx \ge b$. By drawing a segment between any point in $Q' \backslash Q$ and any point in $Q$, we can then argue there is a point in $Q'$ such that $dx=b$.
%%
%%		
%	\end{proof}

	To further understand half-open polyhedra, we note that If $P'$ is a shaving of a polyhedron $P$ with dimension $\ge 1$, then we note that $relint(P) \subseteq P' \subseteq P$, where $relint(P)$ is the relative interior of $P$. This then means that the topological closure of $P'$ is equal to $P$.

	The \emph{face lattice} of a half-open polyhedron $P$ is the set of faces of $P$ ordered under inclusion. We define combinatorial isomorphism the same for half-open polyhedra as for polyhedra, but note that it behaves very differently. 
	
	\begin{definition}
	Two half-open polyhedra $P, P'$ are \emph{combinatorially isomorphic} if their face posets are related by a dimension-preserving isomorphism.
	\end{definition}

	Whereas we can typically imagine that every combinatorial isomorphism between polyhedra can be realized by a homeomorphism, this is not the case for half-open polyhedra. Figure \ref{fig:unintuitive-isomorphism} shows two half-open polyhedra, each a hexagon with four vertices shaved off. The two half-open polyhedra are combinatorially isomorphic, even if any combinatorial isomorphism would have to permute the order of the faces on the boundary. Figure \ref{fig:half-open-isomorphism}, on the other hand, shows a more intuitive example of combinatorially isomorphic half-open polyhedra; one case where we have shaved two sides off a square, one case where we have shaved one side from a triangle, and one cone.

	\begin{figure}
	\centering
	\includegraphics[width=.75\textwidth]{Chapter-3/figs/unintuitive-combinatorial-isomorphism.pdf}
	\caption{A surprising combinatorial isomorphism.}\label{fig:unintuitive-isomorphism}
\end{figure}

	\begin{figure}
	\centering
	\includegraphics[width=.75\textwidth]{Chapter-3/figs/combinatorial-isomorphism.pdf}
	\caption{Three combinatorially isomorphic half-open polyhedra}\label{fig:half-open-isomorphism}
\end{figure}

	A \emph{simple} half-open polyhedron is a half-open polyhedron such that every codimension-$k$ face is contained in $k$ facets. We note that every shaving of a simple polyhedron is a simple half-open polyhedron. The \emph{dual simplicial complex} of a half-open polyhedron $P$ is a simplicial complex such that if $F_s$ for $s \in \mathcal{S}$ is the facet set of $P$, then $I$ is in the dual simplicial complex of $P$ if and only if $\bigcap_{s \in I} F_s \ne \emptyset$. These definitions are identical to those for polyhedra.




	We include the next definition for clarity.

	\begin{definition}
		For a simple polyhedron $P$ defined by facet-defining inequalities $c_i x \le a_i$ for each facet $F_1,\ldots,F_k$ of $P$, the polyhedron defined by the \emph{removal} of a facet $F_j$ from $P$ is the polyhedron defined by inequalities $c_ i x \le a_i$ where $i \ne j$.
	\end{definition}

	Figure \ref{fig:facet-removal} demonstrates the difference between shaving by a facet, and removal of a facet. We note that the combinatorial type of the removal of a facet depends on the angle of adjacent facets, and not just the combinatorial type of the facet. For most polytopes, we can define a projective transformation for each facet such that the shaving of that facet is isomorphic to the removal of that facet. However, this is not possible for unbounded polyhedra or shaving multiple facets. 



Figure \ref{fig:half-open-polyhedra} shows a case where the shaving of several facets gives a half-open polyhedron is not combinatorially isomorphic to any polyhedron.
	
	\begin{figure}[h]
	\centering
	\includegraphics[width=.75\textwidth]{Chapter-3/figs/facet-removal.pdf}
	\caption{A pentagon, the shaving of the pentagon by a facet, and the removal of that facet.} \label{fig:facet-removal}
\end{figure}

	\begin{figure}[h]
	\centering
	\includegraphics[width=.5\textwidth]{Chapter-3/figs/impossible-hexagon.pdf}
	\caption{From left to right: a square, a shaving of the square by a facet, and a combinatorially isomorphic polyhedron obtained by removing a facet from the square.} \label{fig:half-open-polyhedra}
\end{figure}

	\begin{proposition} \label{prop:shaved-simplex}
		When $P$ is an $n$-dimensional simplicial complex, the shaving of $P$ by a facet is an $n$-dimensional simplicial cone.
	\end{proposition}

	This operation can be visualized on the forbidden subset diagram of a simplex. Figure \ref{fig:shaving-forbidden-subsets} shows that the shaving of a facet $F$ removes the facet $F$ from the forbidden subset diagram, as well as the forbidden subset containing $F$, but not the rest of the vertices in the forbidden subset.

\begin{figure}[h]
	\centering
	\includegraphics[width=.75\textwidth]{Chapter-3/figs/shaving-forbidden-subsets.pdf}
	\caption{From left to right: a square, a shaving of the square by a facet, and a combinatorially isomorphic polyhedron obtained by removing a facet from the square.} \label{fig:shaving-forbidden-subsets}
\end{figure}

	The motivation behind all of this discussion of half-open polyhedra comes in the following proposition.

	\begin{proposition}
		When $P$ is a simple polyhedron with facet index set $\mathcal{S}$, and $X \subseteq \mathcal{S}$, the shaving of $P$ by all facets $F_s$ for $s \in X$ has a dual simplicial complex equal to $\Delta(P)\backslash X$.
\end{proposition}

	\begin{proof}
		Shaving by a facet $F_s$ removes all faces contained in that facet, which is analogous to removing any face $S$ of $\Delta(P)$ which contains $s$. We repeat this for every element $s \in X$.
	\end{proof}

	We can then refer to the half-open polyhedron obtained by shaving $P$ by a facet set $X$ as $P \backslash X$. We note that $P \backslash X$ is not always combinatorially isomorphic to a polyhedron. However, Proposition \ref{prop:shaved-simplex} shows that the shaving of a single facet from a simplex is isomorphic to a polyhedron, and it is trivial to show that the shaving of a set of facets from a product of simplices is isomorphic to a simple polyhedron that is the product of rays and simplices. Most importantly for our application, the shaving of any hypercube is isomorphic to the product of a set of $1$-simplices and rays.

	\subsection{$\p$-graph case}

	We will apply Proposition \ref{prop:maximal-tube-enumeration-big-result} to the $\p$-graph case, for a set of families of simplicial complexes $\Delta', A', B', C'$, such that each complex is polyhedral, and that each complex indexed by $n$ is dual to an $n$-dimensional pointed polyhedron. We can rewrite Proposition \ref{prop:maximal-tube-enumeration-big-result} with a change of variables:

	\begin{align*}
	f^{\nest{G_n}{P(\Delta_n')}}(x,y) - \epsilon_L+\epsilon_R =& f^{P(C')}(x,y) (xy)^\rho +  \\
&y \sum_{\sigma \in S} (xy)^{\gamma_\sigma} \sum_{j=1}^k O_y^{A',\sigma,j}[f^{A'^\sigma}(x,y)] O_y^{B',\sigma,j}[f^{B^\sigma'}(x,y)]
\end{align*}


%{	\[
%		f^{\nest{G_n}{P(\Delta_n')}}(x,y) - \epsilon_L+\epsilon_R = f^{P(C')}(x,y) (xy)^\rho + 
%	\]
%	\[
%		y \sum_{\sigma \in S} (xy)^{\gamma_\sigma} \sum_{j=1}^k O_y^{A',\sigma,j}[f^{A'^\sigma}(x,y)] O_y^{B',\sigma,j}[f^{B^\sigma'}(x,y)].
%		\]}

	Now, if we wish to write this, where $\Delta_n$ is the tubing complex of $P_n$-graph $G_n$, and $A, B, C$ are families of $\p$-graphs, we get the following proposition.

	\begin{proposition}
		For a family $P$ of simple polyhedra, $G$ a family of $P$-graphs, and $X_n$ a family of kingmaker sets for each $P_n$-graph $G_n$, consider a family of graphs $A, B$ with shapes $\sigma \in S$ such that for each tube $t$ of shape $\sigma$ with $i+1$ vertices, $A_i^\sigma$ is isomorphic to the simplex-graph associahedron of $G|_t$, and $B_{n-1-\gamma_\sigma-i}^\sigma$ has a dual simplicial complex isomorphic to the $n-1-\gamma_\sigma-i$-dimensional graph associahedron of the neighborless complement of $t$ on the half-open polyhedron obtained by shaving $xn(t)$ from the face $F_t$ of $P_n$. Assume that tubes of shape $\sigma$ are counted by the function $r_\sigma(n,i)$ and is written as a sum of separable functions of the form $r_\sigma^{A,j}(i)r_{\sigma}^{B,j}(n-1-i-\gamma_\sigma)$. Finally, write that the dual simplicial complex of $C_{n-\rho}$ is isomorphic to $\mathcal{N}(G_n\backslash X_n, \Delta(P_n)\backslash X_n)$ for a fixed $\rho$. When $\rho \le 1$, we find

	\[
		f^{P}(x,y)-\epsilon_L = f^{C}(x,y) (xy)^\rho +
		y\sum_{\sigma \in S} (xy)^{\gamma_\sigma} \sum_{j=1}^k
		O_y^{A,\sigma,j}\left[f^{A^\sigma}(x,y)\right]
		O_y^{B,\sigma,j}\left[f^{B^\sigma}(x,y)\right].
	\]
	\end{proposition}

	\begin{proof}
	We simply apply Proposition \ref{prop:maximal-tube-enumeration-big-result} to the $\p$-graph case, by selecting a set of families of polyhedra $P, A, B, C$ and $P$-graphs $G$, such that each polyhedron $P_n, A_n^\sigma, B_n^\sigma, C_n$ is pointed and $n$-dimensional. We then find the complexes $\mathcal{N}(G_n,P_n), \Delta(A_n), \Delta(B_n), \Delta(C_n)$ are all rank $n$, and give us

	\begin{align*}
		f^{\mathcal{N}(P_n,G)}(s,t)-\epsilon_L+\epsilon_R
		=&
		f^{\Delta(C_n)}(s,t)t^\rho +\\
		&st\sum_{\sigma \in S} t^{\gamma_\sigma} \sum_{j=1}^k
		O_t^{A,\sigma,j}\left[f^{\Delta(A)^\sigma}(s,t)\right]
		O_t^{B,\sigma,j}\left[f^{\Delta(B)^\sigma}(s,t)\right].
	\end{align*}

	We then perform a change of variables $s=1/x, t=xy$, and note that $\epsilon_R=0$ when $\rho \le 1$.
\end{proof}

	\begin{remark}
	We should note here that when $\rho \ne 0$, we shave the polyhedron $P_n$ by the set of facets indexed by $X_n$. Call this half-open polyhedron $P_n \backslash X_n$. We note that $P_n \backslash X_n$ is $n$-dimensional, and that $\Delta(P_n)$ is rank $n$, but it is possible that the rank of $\Delta(P_n\backslash X_n)$ is lower than $n$ even if $P_n \backslash X_n$ is $n$-dimensional. We assume that it is rank $n-\rho$ for some constant $\rho$ for all $n \ge \rho$. In this case, we will define the family of polyhedra $C_{k}$ for $k \ge 0$ such that each $C_k$ is $k$-dimensional and the dual simplicial complex of $C_{n-\rho}$ is isomorphic to the complex $\mathcal{N}(G_n \backslash X_n, P_n \backslash X_n)$. As a result, we see that the dual simplicial complex of $C_{n-\rho}$ is $(n-\rho)$-dimensional, even though its dual simplicial complex is isomorphic to the dual simplicial complex of an $n$-dimensional polyhedron. As an example of what this looks like in the hypercube case, see Figure \ref{fig:shaving-dimension} which illustrates the case where $P_2$ is a square, and $X_2$ corresponds to a pair of opposing facets. We see that $P_2 \backslash X_2$ is no longer pointed, and $P_2 \backslash X_2$ is isomorphic to the product of a line and a 1-simplex. As an operation on forbidden subset diagrams, we see this as removing vertices $1$ and $-1$ from the graph, leaving the forbidden subset diagram on $\{2,-2\}$. This diagram is isomorphic to the forbidden subset diagram of just a $1$-simplex, and this is why we define $C_{2-1}$ as a graph associahedron on a $1$-simplex.
\end{remark}

\begin{figure}[h]
	\centering
	\includegraphics[width=.5\textwidth]{Chapter-3/figs/shaving-dimension.pdf}
	\caption{From left to right: a square, a shaving of the square by a facet, and a combinatorially isomorphic polyhedron obtained by removing a facet from the square.} \label{fig:shaving-dimension}
\end{figure}


%, and assume it is isomorphic to a simple polyhedron, such that the $\p$-graph associahedron of the graph $G_n\backslash X_n$ on this polyhedron has a dual simplicial complex isomorphic to $C_{n-\rho}$. We assume that $C_{n-\rho}$ is an $(n-\rho)$-dimensional polyhedron.  
%
%
%the half-open polyhedron 
%
%$C_{n-\rho}$ 


%Set up a series of vertex sets $X_n \subset G_n$ satisfying the terms of the above method. We decompose the tubing complexes of $\mathcal{N}(P_n,G_n)$ again, and et cetera..........
%
%	Define $(C_0,C_1,\ldots)$ to be $\p$-graph associahedra of the shavings of $P_n$ by the facet set $X_n$. Note that as defined, each polyhedron $C_n$ is $n$-dimensional, not $n-\rho$-dimensional.
%
%	Define $\{A_i^\sigma,B_i^\sigma\}_{\sigma \in S, i \ge 0\}$ such that, when $t$ is a tube containing $i+1$ elements in $G_n$ of shape $\sigma$, the maximal tubing complex of $t$ is isomorphic to the dual simplicial complex of the product of polyhedra $A_i^\sigma$ and $B_{n-1-\gamma_\sigma-i}$.
%
%	
%
%	We use the change of variables $s=1/x$ and $t=xy$ to write
%
%	\[
%		f^{\mathcal{N}(P,G)}(x,y)-\epsilon_L = f^{C}(x,y) (xy)^\rho +
%		y\sum_{\sigma \in S} (xy)^{\gamma_\sigma} \sum_{j=1}^k
%		O_y^{A,\sigma,j}\left[f^{A^\sigma}(x,y)\right]
%		O_y^{B,\sigma,j}\left[f^{B^\sigma}(x,y)\right].
%	\] \danger{DOUBLE CHECK THIS! DOUBLE CHECK THIS! OOHGA BOOGAH}
%
%	In the 

%	\subsection{yafhaeha}
%
%	\danger{balewwkhrwejrhe}
%
%	%We now find that we can partition $\mathcal{N}(\Delta_n,G_n)$ into 
%
%	In Section \ref{sec:method-one}, there is an implicit assumption that the rank of an atomic link of a simplicial complex is one less than the rank of the original complex, and that is because we developed this method for pure simplicial complexes. In contrast, it is possible for the rank of a simplicial complex to either change or stay the same after element deletion. As a result, in order to develop a standardized theory, we must introduce variables
%
%	Consider the case where we are calculating the bivariate $f$-polynomial of a family $\{N(\Delta_i,G_i)|i \in \mathbb{N}\}$, where each complex $\Delta_n$ is of rank $n$. Choose a family of vertex subsets $X_0, X_1, \ldots$ such that $X_n$ is a subset of the vertex set of $G_n$, and for any two strongly compatible tubes $t_1, t_2$ such that $t_1 \cap X_n \ne \emptyset, t_2 \cap X_n \ne \emptyset$, we find $t_1\subset t_2$ or $t_2 \subset t_1$. Note that any clique of $G_n$ satisfies this condition.
%
%	Sort the tubes in $intset_{X_n}$ into shapes $\sigma \in S$ such that, for each tube $t$ of $G_n$ and shape $\sigma$ and size $i+1$, the simplex-graph tubing complex of $G_n|_t$ is isomorphic to a simplicial complex $A^\sigma_i$, and the tubing complex $N((G/t)\backslash xn(t),(\Delta/t)\backslash xn(t))$ is isomorphic to some simplicial complex $B^\sigma_{n-1-i-\gamma}$. Write the function $r_\sigma(n,i)$ to count the number of tubes of shape $\sigma$ of size $i+1$ in $intset_{X_n}$.
%
% Furthermore, assume that $N(\Delta_n \backslash X_n, G_n \backslash X_n)$ is isomorphic to a simplicial complex $C_{n-\rho}$.
%
%	We then find that
%
%	\[
%		f^{N(\Delta_n,G_n)} (s) = f^{C_{n-\rho}}(s) + \sum_{\sigma \in S}
%		\sum_{i=0}^{n-1-\gamma}
%		r_\sigma(n,i)
%		f^{A^\sigma_i} (s)
%		f^{B^\sigma_{n-1-\gamma-i}}(s)
%	\]
%
%	Assume again the operators $O^{A^\sigma}_t$ and $O^{B^\sigma}_t$ if separable. We find multiplication by $t^n$ and summation over $n$ gives the following equation:
%
%	\[
%		f^{N(\Delta,G)} (s,t) = f^C(s,t) t^\rho + st (t^\gamma) \sum_{\sigma \in S} O_t^{A^\sigma}\left[f^{A^\sigma}(s,t)\right] O_t^{B^\sigma} \left[f^{B^\sigma}(s,t)\right]
%	\]
%
%	In the case where $\Delta_n$ is the set of dual complexes of hypercubes, we find that all deletion and reconnected complement operations on hypercubes are dual complexes of products of hypercubes and rays.



%	\subsubsection{Example}
%
%	Consider the case of the path simplex graph on $[n+1]$. Set the vertex $1$ as the sole member of our clique $X_n$.The set $\Delta\backslash X$ is just the path graph on $\{2,\ldots,n+1\}$, on a Boolean lattice of $[n+1]\backslash[1]$. Note that this Boolean lattice is dual to an $n$-dimensional simplicial cone, giving us $\rho=0$. \danger{What exactly is Delta here should be rewritten probably...}
%
%	For each $0 \le i \le n-1$, there is exactly one tube $[i+1]$ of size $i+1$ in $X_n$, giving $r(n,i)=1$. The simplex-graph tubing complex of $G|_{[i+1]}$ is the tubing complex of the path simplex graph on $[i+1]$. The neighborless complement $(G\backslash[i+1])\backslash xn([i+1])$ is the path graph on vertices $\{i+3, \ldots, n+1\}$. The link of $[i+1]$ in the dual simplicial complex of the $n$-simplex is the dual simplicial complex of an $n-1-i$-dimensional simplex. Removing $xn([i+1])=\{i+2\}$ from this simplicial complex gives the Boolean lattice on $[n+1]\backslash [i+2]$, which is the dual simplicial complex of an $n-1-i$-dimensional simplicial cone. From these dimensions, we see $\gamma=0$.
%
%	Write that $A_n$ is the $n$-dimensional simplex path graph associahedron, and $P_n$ is the $n$-dimensional simplicial cone path graph associahedron. We write $f^{\Delta(P)} = t f^{\Delta(A)} + \frac{1}{1-st}$.
%
%	Plugging this in, we get
%
%	\[
%		f^{\Delta(A)} = f^{\Delta(P)} + st (f^{\Delta(A)}) (f^{\Delta(P)})
%	\]
%
%	This becomes
%
%	\[
%		f^{\Delta(A)} = t f^{\Delta(A)} + \frac{1}{1-st} + st\left(f^{\Delta(A)}\right)\left(t f^{\Delta(A)} + \frac{1}{1-st}\right)
%	\]	
%
%
%	\subsubsection{Example}
%
%	Consider the case of the path simplex graph on $[n+1]$. Set the vertex $1$ as the sole member of our clique $X$. The set $intset_X$ contains the tubes $\{1\}, \{1,2\},\ldots, [n+1]$. The set $\Delta\backslash X$ is just the path graph on $\{2,\ldots,n+1\}$, on a Boolean lattice of $[n+1]\backslash\{1\}$.
%
%	For each $0 \le i \le n-1$, there is a tube $[i+1]$ in $intset_X$. The simplex graph tubing complex of $G$ restricted to $[i+1]$ is the tubing complex of the $i$-dimensional path graph.
%
%	Assume $A_n$ is the family of path simplex graph asociahedra. Assume that $P_n$ is the family of path simplicial-cone graph associahedra. Note that $f^{\Delta(P)}(s,t)= t f^{\Delta(B)}(s,t)+\frac{1}{1-st}$.

	

%
%
%	Assume that there are sets of simplicial complexes $A_i^\sigma, B^\sigma_i$, such that 
%
%	Assume that there is a collection of shapes $\sigma \in S$ such that there are $r_\sigma(n,i)$ tubes of shape $A^\sigma_i$ which contain $i+1$ vertices in $intset_{X_n}$, and that the tubing complex of the reconnected complement of each tube of shape $\sigma$ and size $i+1$ in $N(\Delta\backslash xn(t), G \backslash xn(t))$ is isomorphic to the simplicial complex $B^\sigma_{n-1-i-\gamma}$.
%
%	We then find
%
%	\[
%		f^{N(\Delta_n,G_n)}(s) = f^{N(\Delta_n\backslash X_n, G_n \backslash X_n)} + \sum_{\sigma \in S} \sum_{i=0}^{n-1} s r_\sigma(n,i) f^{A^\sigma_i}(s) f^{B^\sigma_{n-1-i}} (s)
%	\]

	

%	\begin{figure}
%	\centering
%	\includegraphics[width=.5\textwidth]{example-image-a}
%	\caption{Elimination of one vertex in the hypercube-graph case is equivalent to removing a set of facets from the hypercube-graph associahedron.}
%\end{figure}

%\subsection{Enumerating simplicial complex by partition into relative ideals}
%
%	Every simplicial complex 
%
%
%
%	The $f$-vectors of simplicial complexes can be calculated recursively if there exists a relative ideal decomposition whose components are all isomorphic to simplicial complexes with known $f$-vectors.
%
%	One way to define a relative ideal of a tubing complex is to take two sets of tubes, one set $T_{in}$ of mandatory tubes and one set $T_{out}$ of forbidden tubes, and define the relative simplicial complex of all tubings which contain every tube in $T_{in}$ and do not contain any tube in $T_{out}$. Write such a relative ideal as $(T_{in},T_{out})$.
%
%	\begin{proposition}
%		Consider a set $C$ of vertices in a $\Delta$-graph $G$ such that for no two vertices $v, v' \in C$ we have $\{\{v\},\{v'\}\}$ a valid tubing. If $\mathcal{T}$ is the set of tubings of $G$, define a set of relative ideals of the tubing complex of $G$ as the set of relative ideals $\left( t, \{t' \in \mathcal{T}:t \subsetneq t'\}\right) $ for all $t$ in $T$ containing at least one vertex of $C$, and the set $\left( \emptyset, \right)$
%\end{proposition}
%
%
%
%Given a tube $t$ in a $\Delta$-graph $(G,\Delta)$, we can say that a tube is maximal in a tubing $T$ if $t$ is not a proper subset of any other tube in $T$. We plan to count every tubing of a graph exactly once by choosing a collection of tubes such that no two tubes in this collection are disjoint and compatible, and such that any tubing not containing one of these tubes must avoid a set of vertices entirely.
%
%\begin{definition}
%The \emph{neighborless complement} of a tube $t$ in a $\Delta$-graph $(G,\Delta)$, where $\Delta$ has only disjoint circuits of size $\le 2$, is the $\Delta'$-graph obtained by removing all vertices in $t$, all vertices in $-t$, and all vertices adjacent to vertices in $t$. By keeping all dashed edges between pairs left in the graph, we find that this is the $\p$-graph of a product of rays and $1$-simplices.
%\end{definition}
%
%\begin{proposition}
%If $t$ is maximal in $T$, then $T$ is equal to the union of $t$, $T$ restricted to $t$, and $T$ restricted to the neighborless complement of $t$.
%\end{proposition}
%
%Given a single vertex $i$ in $\pm[n]$ and a tube circuit graph $G$, we can list all the tubes containing $i$. Every tubing either contains $i$ in its support, and therefore contains a maximal tube containing $i$, or does not contain the vertex $i$ in its support.
%
%Here, we will use a new notation. While we used $f^P_{n,k}$ to represent the number of faces of dimension $k$ of a $\p$-graph associahedron $P_n$, we will use the notation $P(n,k)$ to represent the number of tubings of the associated $n$-dimensional $\p$-graph with $k$ tubes.
%
%We will now attempt to count $P(n,k)$. Consider our strategy of splitting tubings by the maximal tube containing $i$. The set of tubings whose supports do not contain $i$ form a graph from $G$ obtained by removing the vertex $i$ from the tube circuit graph of $G$. This resulting graph is a tube circuit graph of dimension either $n$ or $n-1$. We count this by either $C(n,k)$ or $C(n-1,k)$, which we can rewrite as $C(n-\rho,k)$.
%
%Now for a tube $t$ of shape $s$ containing $k+1$ elements, say that the tube induces a graph of type $A^s$ and the neighborless complement is a graph of type $B^s$. The graph of $A^s$ will be known to give a $k$-dimensional graph associahedron, but the $B^s$-type graph likely involves removing a large number of vertices, and will be $n-1-i-\gamma$-dimensional, for some $\gamma \ge 0$. If there are $t_s(n,k)$ tubes of shape $s$ containing $k+1$ elements, then we calculate the following:
%
%\[
%	f^{\Delta_n}_k = f^{C_{n-\rho}}_k + \sum_{\sigma \in S} \sum_{i=0}^{n-1} \sum_{j=0}^{k-1} r_\sigma(n,i) f^{A^\sigma_i}_j f^{B^\sigma_{n-1-i-\gamma}}_{k-1-j}
%\]
%
%We can take summation over all $n, k \ge 0$. This yields
%
%\[
%	\sum_{n,k\ge 0} f^{\Delta_n}_k s^k t^n =\sum_{n,k \ge 0} \left( f^{C_{n-\rho}}_k s^k t^{n-\rho} t^\rho
%	+\sum_{\sigma \in S} \sum_{i=0}^{n-1} \sum_{j=0}^{k-1} r_\sigma(n,i) f^{A^\sigma_i}_j (s^j t^i)  f^{B^\sigma_{n-1-i-\gamma}}_{k-1-j} (s^{k-1-j} t^{n-1-i-\gamma}) s t^{1+\gamma}
%	\right)
%\]
%
%This turns into
%
%\[
%	f^\Delta(s,t) = f^C(s,t) t^\rho + st^{1+\gamma} \sum_{\sigma \in S} O_t^{A^\sigma}\left[ f^{A^\sigma}(s,t) \right] O_t^{B^\sigma}\left[ f^{B^\sigma}(s,t) \right]
%\]
%
%\danger{And maybe with a +1 in there??? Or an optional +1?}
%
%
%
%\danger{This is still not a comprehensive general form for this formula, and we will continue to adapt it for other generating functions. However, this is good for now. We do, however, have to rewrite this all in terms of generating functions, which means we have to reparameterize, starting by switching $k$ with $n-k$.}
%
%\[
%	P(n,n-k) = C(n-\rho,n-k) + \sum_{s \in S} \sum_{i=0}^{n-1} \sum_{j=0}^{n-k-1} t_s(n,i) A^s(i,j) B^s(n-1-i-\gamma,n-k-1-j)
%\]
%
%\pagebreak

==> Chapter-6/Chapter-6.tex <==
\chapter{CONCLUSIONS}
\label{chap:conc}

% Example headers
\section{Summary of Results}
\label{sec:summ}


\section{Overarching Conclusions}
\label{sec:conc}


\section{Future Work}
\label{sec:future}


==> Chapter-Other/Chapter-Other.tex <==
\chapter{Summary of Future Work}
\label{chap:other}

%\section{$\p$-Nestohedra as Sections of Simplex-Nestohedra}\label{sectionsection}
%
%	\danger{Alternate titles: $\p$-Nestohedra as intersections of Nestohedra and generic subspaces... Do I want to bring generic-ness into it?}
%
%	It is well known that every polytope is isomorphic to the intersection of an affine subspace and a higher dimensional simplex. In this section, we show that every $\p$-nestohedron, where $\p$ is $n$-dimensional and has $k$ facets, is isomorphic to the intersection of an $n$-dimensional affine subspace with a $k$-dimensional nestohedron.
%
%%	\danger{I am not entirely sure of the correct framing here.}
%%
%%	The paper \cite{intervalstretching} describes a dual process to our paper, wherein we can define a building set and nested complexes for a simple polytope.
%%
%%	Every simplicial complex can be defined naturally as a subset of a boolean lattice...
%
%	\begin{definition}
%		Let $\p$ be a simple $n$-dimensional polytope in $\R^n$ with facets $F_1, \ldots, F_k$ and faces $F_I=\bigcap_{i \in I} F_i$. Define $\Delta$ to be a simplex with facets $D_1,\ldots, D_k$ and faces $D_I=\bigcap_{i \in I} D_i$. For any $\Delta$-building set $\B$, define $\B|_\p$ as the $\p$-building set defined by $\{S \in \B: F_S \ne \emptyset\}$. For any $\p$-building set, define $\B|^\Delta$ to be the smallest $\Delta$-building set containing $\B$.
%	\end{definition}
%
%		The building set $\B|^\Delta$ is well-defined because the intersection of any two building sets is still a building set. Also note that for a $\p$-building set $\B$, $\B =(\B|^\Delta) |_\p$, but for a $\Delta$-building set $\B$, we find $\B$ is not necessarily equal to $(\B|_\p )|^\Delta$. The following proposition describes the relationships between the nested complexes of these building sets.
%
%	\begin{proposition}
%		Given a simplex-building set $\B$ indexed on $[k]$, and a simple polytope $\p$ with $k$ facets $F_1,\ldots, F_k$, the nested complex of $\B|_\p$ is the set of nested sets $N$ under $\B$ such that $F_{\support{N}} \ne \emptyset$.
%	\end{proposition}
%
%	The nested complex of $\B|_\p$ is a subcomplex of the nested complex of $\B$. The following lemma and theorem show that we can realize this complex geometrically, expressing $\nest{\p}{\B}$ as the intersection of a subspace and $\nest{\Delta}{\B}$. \danger{should probably write the theorem first, and then the lemma and proof.}
%	
%
%
%	\begin{lemma} \label{intersectionlemma}
%		Every $n$-dimensional simple polytope $\p$ with facets $F_1,\ldots,F_k$ is affinely isomorphic by map $\phi$ to the intersection of an $n$-dimensional subspace $U$ and a simplex with facets $D_1,\ldots,D_k$ and intersections labeled $D_S=\bigcap_{i \in S}D_i$ such that $U \cap D_i=\phi(F_i)$.
%	\end{lemma}
%
%	\begin{proof}
%		The fact that $\p$ must be affinely isomorphic to the intersection of a subspace and a standard simplex is well-known, and is a statement dual to the fact that every polytope is affinely isomorphic to a projection of a simplex. There exists a representation of $\p$ by an inequality $Ax - b \ge 0$, where each inequality $a_ix -b_i \ge 0$ defines a facet. The map $\phi:x \mapsto Ax - b$ defines a subspace $U=\phi(\R^n)$ containing a polytope $\phi(\p)$ affinely isomorphic to $\p$. The subspace $U$ is contained in some hyperplane $H=\{y\in \R^k:cy=-cb\}$ with positive row vector $c$, and define $\Delta=H\cap \R^k_{\ge 0}$.
%
%		The set $U \cap D_i$ is the image of elements $x \in \p$ such that $a_i x - b_i = 0$. This is exactly the image of $F_i$ under $\phi$, proving the lemma.
%	\end{proof}
%
%\danger{a note about notation}
%
%	\begin{theorem}
%		Given a simplex $\Delta$ with $k$ facets, a $\Delta$-building set $\B$, and a simple $n$-dimensional polytope $\p$ with $k$ facets, there is a realization of $\nest{\Delta}{\B}$ and an $n$-dimensional affine subspace $U$ such that $U \cap \nest{\Delta}{\B}$ is isomorphic to $\nest{\p}{\B|_\p}$.
%	\end{theorem}
%
%\begin{proof}
%
%Order the elements of $\B = \{\{1\},\ldots,\{k\}, S_1, \ldots, S_m\}$ such that if $S_i \subset S_j$, then $i > j$. Define $\B_i = \{\{1\},\ldots,\{k\},S_1,\ldots,S_i\}$. For ease of notation, for a set $S$, define $S^*=\{\{s\}:s \in S\}$.
%The polytope $\nest{\Delta}{\B_0}$ is equal to the simplex $\Delta$, and $\nest{\Delta}{\B_i}$ is obtained by truncating the face $D(S_i^*,\B_{i-1})$ in the polytope $\nest{\Delta}{\B_{i-1}}$, by a certain depth. 
%
%Note that because the face $D_{S_i}$ has not yet been truncated in this truncation order, we get \[D(S_i^*,\B_{i-1})=D_{S_i} \cap \nest{\Delta}{\B_{i-1}}.\] This face is defined by the inequality $e_{S_i} \cdot x - b \ge 0$. \danger{this face is defined by the inequality should really be reworded...}
%
%As an inductive step, assume that the intersection $U \cap \nest{\Delta}{\B_{i-1}}$ is isomorphic to $\nest{\p}{(\B_{i-1}|_\p)}$. We wish to prove that $U \cap \nest{\Delta}{\B_{i}}$ is isomorphic to $\nest{\p}{(\B_{i}|_\p)}$. If $S_i \notin \B_{i}|_\p$, then $\B_{i}|_\p=\B_{i-1}|_\p$ the face $F_{S_i}=D_{S_i} \cap U$ is empty. This means that the face
%$D(S_i^*,\B_{i-1})$ does not intersect with $\nest{\p}{(\B_{i-1}|_\p)}$. As a result, we can choose a sufficiently shallow hyperplane $e_{S_i} \cdot x \ge \varepsilon$ which separates the face $D(S_i^*,\B_{i-1})$ from $\nest{\p}{(\B_{i-1}|_\p)}$. By truncating $\nest{\Delta}{\B_{i-1}}$ by this polytope, we get $\nest{\Delta}{\B_i}$. However, this hyperplane misses $\nest{\p}{(\B_{i-1})}$ entirely, leaving that polytope unchanged.
%
%If, on the other hand, $S_i \in \B_{i}|_\p$, then we want to choose a sufficiently shallow hyperplane which truncates both $\nest{\Delta}{\B_{i-1}}$ and $\nest{\p}{(\B_{i-1}|_\p)}$. We know that $D_{S_i} \cap U$ is nonempty. We find that the face $D(S_i^*,\B_{i-1})$ of $\Delta$ is defined by the inequality $e_{S_i} \cdot x \ge 0$, and we find that $D(S_i^*,\B_{i-1}) \cap U = \face{S_i^*}{\B_{i-1}|_\p}$. As a result, we find that $\face{S_i^*}{\B_{i-1}|_\p}$ is defined by the hyperplane $e_{S_i} \cdot x \ge 0$. As a result, we just need to pick sufficiently small $\varepsilon > 0$ such that $e_{S_i} \cdot x \ge 0$ truncates both faces, which can be done by taking the minimum of the $\varepsilon$ value needed to truncate either face.
%
%As a result, we find that $U \cap \nest{\Delta}{\B_i}$ is isomorphic to $\nest{\p}{(\B_{i-1}|\p)}$.
%\end{proof}
%
%For a given $\p$-building set $\B$, we know that $\B=(\B|^\Delta)|_\p$, which yields the following corollary.
%
%\begin{corollary}
%Given an $n$-dimensional simple polytope $\p$ with $k$ facets, and a building set $\B$, the $\p$-nestohedron $\nest{\p}{\B}$ is linearly isomorphic to the intersection of an $n$-dimensional subspace and a nestohedron $\nest{\Delta}{\B|^\Delta}$.
%\end{corollary}
%
%	\begin{example}
%		The hypercube can be expressed as a section of a simplex as follows. If $\Delta_{2n-1}$ is the simplex on $2n$ coordinates $\{x_i:i \in \pm[n]\}$ such that each $x_i \ge 0$ and $\sum_{i \in \pm[n]} x_i = n$, then the intersection of the affine subspace $T = \{x: x_i+x_{-i}=1 \forall i\in[n]\}$ with $\Delta_{2n-1}$ is isomorphic to the standard hypercube; it is the Minkowski sum of the $n$ line segments which are the convex hulls of the pairs $\{e_i,e_{-i}\}$. 
%	\end{example}

==> Makefile <==
CHAPTERS=Chapter-*/Chapter-*.tex  Appendix-*/Appendix-*.tex
NAME=YourName-thesis
AUX=$(NAME).aux front.aux Chapter-*/*.aux Appendix-*/*.aux optional.aux
INTERMEDIATES=$(NAME).bbl $(NAME).blg $(NAME).lof $(NAME).lot \
              $(NAME).log $(NAME).toc 

$(NAME).pdf : $(NAME).tex $(NAME).bib front.tex $(CHAPTERS) ncsuthesis.cls optional.tex
	pdflatex $(NAME)
	bibtex $(NAME)
	pdflatex $(NAME)
	pdflatex $(NAME)

clean :
	rm $(AUX) $(INTERMEDIATES)




==> optional.tex <==
%%  Optional Packages to consider.   These packages are compatible with
%%    ncsuthesis.  

%% -------------------------------------------------------------------------- %%
%% Fancy chapter headings
%%  available options: Sonny, Lenny, Glenn, Conny, Rejne, Bjarne
%\usepackage[Sonny]{fncychap}
\usepackage[Rejne]{fncychap}

%%----------------------------------------------------------------------------%%
%% Hyperref package creates PDF metadata and hyperlinks in Table of Contents
%%  and citations.  Based on feedback from the NCSU thesis editor, 
%%  the links are not visually distinct from normal text (i.e. no change
%%  in color or extra boxes).
\usepackage[
  pdfauthor={Change author in optional.tex},
  pdftitle={Change title in optional.tex},
  pdfcreator={pdftex},
  pdfsubject={NC State ETD Dissertation},
  pdfkeywords={change key words in optional.tex},
  colorlinks=true,
  linkcolor=black,
  citecolor=black,
  filecolor=black,
  urlcolor=black,
]{hyperref}


%% -------------------------------------------------------------------------- %%
%% Microtype - If you use pdfTeX to compile your thesis, you can use
%%              the microtype package to access advanced typographic
%%              features.  By default, using the microtype package enables
%%              character protrusion (placing glyphs a hair past the right 
%%              margin to make a visually straighter edge)
%%              and font expansion (adjusting font width slightly to get 
%%              more favorable justification).
%%              Using microtype should decrease the number of lines
%%              ending in hyphens.
\usepackage{microtype}


%%----------------------------------------------------------------------------%%
%% Fonts 

%% ETD guidelines don't specify the font.  You can enable the fonts
%%  by uncommenting the appropriate lines.  Using the default Computer 
%%  Modern fonts is *not* required.  A few common choices are below.
%%  See http://www.tug.dk/FontCatalogue/ for more options.

%% Serif Fonts -------------------------------------------------
%%  The four serif fonts listed here (Utopia, Palatino, Kerkis,
%%  and Times) all have math support.


%% Utopia
\usepackage[T1]{fontenc}
\usepackage[adobe-utopia]{mathdesign}

%% Palatino
%\usepackage[T1]{fontenc}
%\usepackage[sc]{mathpazo}
%\linespread{1.05}

%% Kerkis
%\usepackage[T1]{fontenc}
%\usepackage{kmath,kerkis}

%% Times
%\usepackage[T1]{fontenc}
%\usepackage{mathptmx}


%% Sans serif fonts -------------------------

%\usepackage[scaled]{helvet}  % Helvetica
%\usepackage[scaled]{berasans} % Bera Sans
